On the complexity of stratified logics

Our primary motivation is the comparison of two different traditions used in ICC to characterize the class FPTIME of the polynomial time computable functions. On one side, FPTIME can be captured by Intuitionistic Light Affine Logic (ILAL), a logic derived from Linear Logic, characterized by the structural invariant Stratification. On the other side, FPTIME can be captured by Safe Recursion on Notation (SRN), an algebra of functions based on Predicative Recursion, a restriction of the standard recursion schema used to defiine primitive recursive functions. Stratifiication and Predicative Recursion seem to share common underlying principles, whose study is the main subject of this work.

==> bib-et-index.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %%%%
  \clearpage  %flushes figures
  \addcontentsline{toc}{chapter}{Index}
  \printindex
  %%%%
%   \clearpage
  \addcontentsline{toc}{chapter}{Table of Symbols}
  \printtos
  %%%%
  \clearpage
  \addcontentsline{toc}{chapter}{Bibliography}
  \bibliographystyle{alpha}
  \bibliography{idee}


==> fig-LINEAR-X.tex <==
\complexfigure
{An example of ramified partial order.
The two contraction nodes show how the modalities influence the construction of the trees of contractions in $\PLTSS{M}$.
}
{fig:example-ramified-po}
{
  \centering
       \proofnetpagescaled[nodesep=2pt,colsep=.3]{\zoomdefault}{0.4\textwidth}{
                        &&              &              &&              &                   &\Rnode{44}{nn}\\ \\
                        &&              &              &&\Rnode{33}{33}&\Rnode{33p}{\cdots}&\Rnode{34}{(n-1)n}\\ \\
                        &&              &\Rnode{22}{22}&
                        %%%%%
                          {\psset{linecolor=red}
                           \nConrot{22b}
                           \nccurve[angleB=90
                                   ,angleA=240
%                                    ,offsetA=9.5pt
                                   ]{33}{22b}
                           \nccurve[angleA=260
                                   ,angleB=-45
                                   ,offsetA=-2pt
                                   ]{22b}{22}
                          }
                        %%%%%
                                               &\Rnode{23}{23}&\Rnode{23p}{\cdots}&\nVoid{24}\\\\
                        &\Rnode{11}{11}&
                        %%%%%
                          {\psset{linecolor=blue}
                           \nConrot{12b}
                           \nccurve[angleA=-90
                                   ,angleB=90
%                                    ,offsetA=9.5pt
                                   ]{22}{12b}
                          }
                        %%%%%
                                               &\Rnode{12}{12}&&\Rnode{13}{13}
                         %%%%%
                          {\psset{linecolor=red}
                           \nccurve[angleA=280
                                   ,angleB=135
                                   ,offsetA=2pt
                                   ]{22b}{13}
                          }
                        %%%%%
                          {\psset{linecolor=blue}
                           \nccurve[angleA=-90
                                   ,angleB=-45
                                   ,offsetA=-2pt
                                   ]{12b}{11}
                           \nccurve[angleA=-90
                                   ,angleB=235
                                   ,offsetA=2pt
                                   ]{12b}{12}
                          }
                        &\Rnode{13p}{\cdots}&\nVoid{14}\\\\
          \Rnode{00}{00}&\Rnode{01}{01}&&\Rnode{02}{02}&&\Rnode{03}{03}&\Rnode{03p}{\cdots}&\Rnode{04}{0n}\\\\
                        &              &\Rnode{b}{\phantom{\sum}\pas\phantom{\sum}}
          %%%%%%%%%%%%%%%%%
          \ncline{-}{b}{00}
          \ncline{-}{b}{01}
          \ncline{-}{b}{02}
          \ncline{-}{b}{03}
          \ncline[linestyle=dashed]{-}{b}{04}
          %%%%%%%%%%%%%%%%%
          \ncline{-}{01}{11}
          \ncline{-}{02}{12}
          \ncline{-}{03}{13}
          \ncline{-}{04}{14}
          %%%%%%%%%%%%%%%%%
          \ncline{-}{12}{22}
          \ncline{-}{13}{23}
          %%%%%%%%%%%%%%%%%
          \ncline{-}{23}{33}
          %%%%%%%%%%%%%%%%%
          \ncline{-}{00}{11}
          \ncline{-}{11}{22}
          \ncline{-}{22}{33}
          \ncline[linestyle=dashed]{-}{33}{44}
          %%%%%%%%%%%%%%%%%
          \ncline{-}{34}{44}
          %%%%%%%%%%%%%%%%%
          \ncline[linestyle=dashed]{-}{14}{34}
          }
} %complexfigure

==> fig-binary-church.tex <==
\complexfigure
{(Church) Words.}
{fig:church-bin-num}
{
\centering
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subfloat[$\ZW$]{
\label{subfig:ZW}
 \proofnetpagescaled[colsep=1cm]{\zoomdefault}{2.5cm}{
  &&\nVoid{out}\\
  &&\nRfor{rfor}\\
  &&\nRlin{lambda1}\\
  &&\nRlin{lambda2}\\
  &&\nPa{port}\\
  &&\nRlin{lambda3}\\
  \nWea{weak1} &\nWea{weak2} &\nAx{ax}\\
  %%%%%%%%%%%%
  \ncline{rfor}{out} \nbput{\NC}
  \ncline{lambda1}{rfor}
%     \nbput{!{(\alpha\lin\alpha)}\lin!{(\alpha\lin\alpha)}\lin\pa{(\alpha\lin\alpha)}}
  \ncline{lambda2}{lambda1}
%   \nbput{!{(\alpha\lin\alpha)}\lin\pa{(\alpha\lin\alpha)}}
  \ncline{port}{lambda2}
    \naput{\pa{(\alpha\lin\alpha)}}
  \ncline{lambda3}{port}
%     \naput{\alpha\lin\alpha}
  \ncline{ax}{lambda3} \nbput{\alpha}
  \ncldownup[armA=25mm]{lambda1}{weak1} \nbput[npos=0.5]{!{(\alpha\lin\alpha)}}
  \ncldownup[armA=15mm]{lambda2}{weak2} \nbput[npos=0.5]{!{(\alpha\lin\alpha)}}
  \ncldownup[armA=1mm]{lambda3}{ax} \nbput[npos=3.5]{\alpha}
  %%%%%%%%%%%%%
  \ncloop[linewidth=1.5pt,linecolor=blue,linestyle=dotted,loopsize=25mm,angleA=180,angleB=0]{-}{port}{port}
  }%proofnetpagescaled
 } %subfigure
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subfloat[\mbox{$\SW_0[w]$}]{
\label{subfig:SW-0}
  \qquad
  \proofnetpagescaled{\zoomdefault}{3.7cm}{
  &\nVoid{out}\\
  &\nRfor{rfor}\\
  &\nRlin{imp1}\\
  &\nRlin{imp1b}\\
  &\nPa{port1}\\
  &\nRlin{imp2}\\
  &\nAx{ax1}\\
  &\nLlin{llin1}\\
  &&\nAx{ax2}\\
  &&\nLlin{llin2}\\
  &&&\nAx{ax3}\\
  &\nOC{pax1}&\nPa{pax2}\\
  &&\nLlin{apply}\\
  \nWea{weak}&&\nLfor{lfor}&\nAx{ax4}\\
  &\nCon{con}\\
  &&\nVoid{input}
  %%%%%%%%%%%%
  \ncline{rfor}{out} \nbput{\NC}
  \ncline{imp1}{rfor}
%     \nbput{!{(\alpha\lin\alpha)}\lin!{(\alpha\lin\alpha)}\lin\pa{(\alpha\lin\alpha)}}
  \ncline{imp1b}{imp1}
%     \nbput{!{(\alpha\lin\alpha)}\lin\pa{(\alpha\lin\alpha)}}
  \ncline{port1}{imp1b} \nbput{\pa{(\alpha\lin\alpha)}}
  \ncline[offset=2pt]{con}{pax1}  \naput{!(\alpha\lin\alpha)}
  \ncangle[offsetA=-2pt,angleA=90,angleB=-90,armB=3mm]{con}{ax4}
  \ncangle[angleA=90,angleB=0]{ax4}{apply}
  \ncldownup[armA=9mm]{imp1}{con} \nbput[npos=0.5]{!{(\alpha\lin\alpha)}}
  \ncldownup[armA=8mm]{imp1b}{weak} \nbput[npos=0.5]{!{(\alpha\lin\alpha)}}
  \ncline{apply}{pax2} \nbput{\pa(\alpha\lin\alpha)}
  \ncline{lfor}{apply} \ncput[npos=0.4]{!{(\alpha\lin\alpha)}\lin\pa{(\alpha\lin\alpha)}}
  \ncline{input}{lfor} \nbput\NC
  %%%inside box:
  \ncline{imp2}{port1} \nbput{(\alpha\lin\alpha)}
  \ncline{ax1}{imp2} \nbput{\alpha}
  \ncline{llin1}{ax1} \nbput{\alpha}
  \ncline{pax1}{llin1} \naput{\alpha\lin\alpha}
  \ncangle[angleA=90,angleB=0]{ax2}{llin1} \nbput[npos=0.5]{\alpha}
  \ncline{llin2}{ax2} \nbput{\alpha}
  \ncline{pax2}{llin2} \naput{\alpha\lin\alpha}
  \ncangle[angleA=90,angleB=0]{ax3}{llin2} \nbput[npos=0.5]{\alpha}
  \ncldownup[armB=2.5mm]{imp2}{ax3} \nbput[npos=3.5]{\alpha}
  %%% box:
  \ncangle[linewidth=1.5pt,linecolor=blue,linestyle=dotted,angleA=180,angleB=180,arm=8mm]{-}{port1}{pax1}
  \ncline[linewidth=1.5pt,linecolor=blue,linestyle=dotted]{-}{pax1}{pax2}
  \ncangle[linewidth=1.5pt,linecolor=blue,linestyle=dotted,angleA=0,angleB=0,arm=25mm]{-}{pax2}{port1}
  }%proofnetpagescaled
 } %subfigure
\subfloat[\mbox{$\SW_1[w]$}]{
\label{subfig:SW-1}
  \qquad
  \proofnetpagescaled{\zoomdefault}{3.7cm}{
  &\nVoid{out}\\
  &\nRfor{rfor}\\
  &\nRlin{imp1}\\
  &\nRlin{imp1b}\\
  &\nPa{port1}\\
  &\nRlin{imp2}\\
  &\nAx{ax1}\\
  &\nLlin{llin1}\\
  &&\nAx{ax2}\\
  &&\nLlin{llin2}\\
  &&&\nAx{ax3}\\
  &\nOC{pax1}&\nPa{pax2}\\
  &&\nLlin{apply}\\
  \nWea{weak}&&\nLfor{lfor}&\nAx{ax4}\\
  &\nCon{con}\\
  &&\nVoid{input}
  %%%%%%%%%%%%
  \ncline{rfor}{out} \nbput{\NC}
  \ncline{imp1}{rfor}
%     \nbput{!{(\alpha\lin\alpha)}\lin!{(\alpha\lin\alpha)}\lin\pa{(\alpha\lin\alpha)}}
  \ncline{imp1b}{imp1}
%     \nbput{!{(\alpha\lin\alpha)}\lin\pa{(\alpha\lin\alpha)}}
  \ncline{port1}{imp1b} \nbput{\pa{(\alpha\lin\alpha)}}
  \ncline[offset=2pt]{con}{pax1}  \naput{!(\alpha\lin\alpha)}
  \ncangle[offsetA=-2pt,angleA=90,angleB=-90,armB=3mm]{con}{ax4}
  \ncangle[angleA=90,angleB=0]{ax4}{apply}
  \ncldownup[armA=9mm]{imp1b}{con} \nbput[npos=0.5]{!{(\alpha\lin\alpha)}}
  \ncldownup[armA=8mm]{imp1}{weak} \nbput[npos=0.5]{!{(\alpha\lin\alpha)}}
  \ncline{apply}{pax2} \nbput{\pa(\alpha\lin\alpha)}
  \ncline{lfor}{apply} \ncput[npos=0.4]{!{(\alpha\lin\alpha)}\lin\pa{(\alpha\lin\alpha)}}
  \ncline{input}{lfor} \nbput\NC
  %%%inside box:
  \ncline{imp2}{port1} \nbput{(\alpha\lin\alpha)}
  \ncline{ax1}{imp2} \nbput{\alpha}
  \ncline{llin1}{ax1} \nbput{\alpha}
  \ncline{pax1}{llin1} \naput{\alpha\lin\alpha}
  \ncangle[angleA=90,angleB=0]{ax2}{llin1} \nbput[npos=0.5]{\alpha}
  \ncline{llin2}{ax2} \nbput{\alpha}
  \ncline{pax2}{llin2} \naput{\alpha\lin\alpha}
  \ncangle[angleA=90,angleB=0]{ax3}{llin2} \nbput[npos=0.5]{\alpha}
  \ncldownup[armB=2.5mm]{imp2}{ax3} \nbput[npos=3.5]{\alpha}
  %%% box:
  \ncangle[linewidth=1.5pt,linecolor=blue,linestyle=dotted,angleA=180,angleB=180,arm=8mm]{-}{port1}{pax1}
  \ncline[linewidth=1.5pt,linecolor=blue,linestyle=dotted]{-}{pax1}{pax2}
  \ncangle[linewidth=1.5pt,linecolor=blue,linestyle=dotted,angleA=0,angleB=0,arm=25mm]{-}{pax2}{port1}
  }%proofnetpagescaled
 } %subfigure
}%complexfigure

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\complexfigure
{Bit reversion over (Church) Words.}
{fig:church-reverse}
{
\centering
\subfloat[\mbox{$\RevW[w]$}]{
\label{subfig:RevW}
 \proofnetpagescaled[colsep=13mm]{\zoomdefault}{4.1cm}{
  \nVoid{o11}\\
  \nRfor{rf31}\\
  \nRlin{rl41}\\
  \nRlin{rl51}\\
  \nPa{rp61  }\\
  \nLlin{ll71 }&\simplenet{id72}{\lambda x.x}\\
  \nPa{lp81  }\\
  \nLlin{ll91 }&\simplenet{st92 }{\texttt{Step}_1}\\
  \nLlin{ll101}\\
  \nLfor{lf111}&\simplenet{st112}{\texttt{Step}_0}\\
  \\ \\
  \nVoid{i121}
  %%%%%%%%%%%
  %first column
  \ncline{rf31 }{o11 }
    \nbput{\NC}
  \ncline{rl41 }{rf31 }
  \ncline{rl51 }{rl41 }
  \ncline{rp61 }{rl51 } \nbput{\S(\alpha\lin\alpha)}
  \ncline{ll71 }{rp61 }
  \ncline{lp81 }{ll71 } \nbput{\alpha\lin\alpha}
  \ncline{ll91 }{lp81 }
  \ncline{ll101}{ll91 }
  \ncline{lf111}{ll101} \nbput{\NC\{\alpha\lin\alpha\}}
  \ncline{i121}{lf111}
    \nbput{\NC}
  % second column
  \ncangle[angleA=90,angleB=45]{id72 }{ll71 } \nbput[npos=1.3]{(\alpha\lin\alpha)\lin(\alpha\lin\alpha)}
  \ncangle[angleA=90,angleB=45]{st92 }{ll91 }
  \ncangle[angleA=90,angleB=45]{st112}{ll101}
  % abstraction links
  \ncangles[angleA=180,angleB=-90,armA=4mm]{rl41}{st112}
  \ncloop[angleA=180,angleB=0,armA=5mm,armB=2mm,loopsize=66mm]{rl51}{st92 }
  %%%%% box
  \ncangle[linewidth=1.5pt,linecolor=blue,linestyle=dotted,angleA=180,angleB=180]{-}{rp61}{lp81}
  \ncangle[linewidth=1.5pt,linecolor=blue,linestyle=dotted,angleA=0,angleB=0,armB=30mm]{-}{lp81}{rp61}
  }%proofnetpagescaled
 } %subfigure
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\qquad
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subfloat[\texttt{Step}${}_i$ with $i\in\{0,1\}$]{
\label{subfig:Step-i}
 \proofnetpagescaled[colsep=1cm]{\zoomdefault}{3.5cm}{
  \nVoid{o11}\\
  \nOC{ro21  }\\
  \nRlin{rl31 }\\
  \nRlin{rl41 }\\
  \nLlin{ll51 }&\nLlin{ll52 }&\nAx{ax53 }\\ \\
               &\nOC{lo62  }\\
               &\nVoid{i72}
  %%%%%%%%%%%%
  % first column
  \ncline{ro21 }{o11 }
    \nbput{!s((\alpha\lin\alpha)\lin \alpha\lin\alpha)}
  \ncline{rl31 }{ro21 }
    \nbput{(\alpha\lin\alpha)\lin \alpha\lin\alpha}
  \ncline{rl41 }{rl31 }
  \ncline{ll51 }{rl41 }
  % second column
  \ncangle[angleA=90,angleB=45]{ll52 }{ll51 }
  \ncangle[angleA=90,angleB=45]{ax53 }{ll52 }
  \ncline{lo62}{ll52}
  \ncline{i72}{lo62}
    \nbput{!s(\alpha\lin\alpha)}
  % abstraction links
  \ncangles[angleA=180,angleB=-90,armA=4mm]{rl31}{ll51}
  \ncangles[angleA=180,angleB=-90,armA=5mm,armB=6mm]{rl41}{ax53 }
  %%%%%%%%%%%%%%% box
    \ncangle[linewidth=1.5pt,linecolor=red,angleA=0,angleB=0,armB=18mm]{-}{ro21}{lo62}
    \ncangle[linewidth=1.5pt,linecolor=red,angleA=180,angleB=180,armB=10mm]{-}{lo62}{ro21}
  }%proofnetpagescaled
 } %subfigure
} %complexfigure



==> fig-church-numerals.tex <==
\complexfigure[!b]
{$\PLTSS{M}$: encoding Church numerals and successor.}
{fig:PLTS-CN-and-succ}
{% CurchNumeralN
\subfloat[A Church numeral less than $m$.]{
\label{subfig:PLTS-CN}
\proofnetpagescaled[rowsep=.1,colsep=1]{\zoomdefault}{.5\textwidth}{
\nOut{a}   \\ \\
\nRfor{b} \\ \\
\nRlin{c} \\ \\
\nRpa{d} \\ \\
\nRlin{e} \\ \\
\nAx{f} \\ \\
\nLlin{gu} & \nAx{gd} \\ \\
           & \nLlin{hu} & \nAx{hd} \\ \\
           &            & \nLlin{iu} & \nAx{id} \\ \\
\nLpa{ju}  & \nLpa{jd}  & \nLpa{jt}  \\ \\
\nCon{ku}   & \nCon{kd}   & \nCon{kt} & \nWea{jq} \\ \\
%%%
\ncline{b}{a}
  \nbput{\forall\alpha.
         {\modm_m}{(\alpha\linear\alpha)}\linear
         \pa{(\alpha\linear\alpha)} = \titiNatT{\modm_m}}
\ncline{c}{b}
  \nbput{{\modm_m}{(\alpha\linear\alpha)}\linear
         \pa{(\alpha\linear\alpha)}}
\ncline{d}{c}
  \nbput{\pa{(\alpha\linear\alpha)}}
\ncline{e}{d}
\ncline{f}{e}
\ncline{gu}{f}
\nccurve[angleA=135,angleB=45]{gd}{gu}
\ncline{hu}{gd}
\nccurve[angleA=135,angleB=45,linestyle=dashed]{hd}{hu}
\ncline{iu}{hd}
\nccurve[angleA=135,angleB=45]{id}{iu}
\ncangles[angleA=180,angleB=-90,armA=.1,armB=.6]{e}{id}
  \nbput{\alpha}
\ncline{ju}{gu}
  \nbput{\alpha\linear\alpha}
\ncline{jd}{hu}
  \nbput{\alpha\linear\alpha}
\ncline{jt}{iu}
  \nbput{\alpha\linear\alpha}
\ncline{ku}{ju}
\nccurve[angleA=45,angleB=-90]{ku}{kd}
  \nbput{\modm_{m-1}{(\alpha\linear\alpha)}}
\ncline{kd}{jd}
\nccurve[angleA=45,angleB=-90,linestyle=dashed]{kd}{kt}
\ncline{kt}{jt}
\nccurve[angleA=45,angleB=-90]{kt}{jq}
  \nbput{\modm_{1}{(\alpha\linear\alpha)}}
\ncangles[angleA=180,angleB=-90,armA=.9]{c}{ku}
  \nbput[npos=2.5]{\modm_m{(\alpha\linear\alpha)}}
% box border
\ncbar[angle=0,arm=2.3,linewidth=1.5pt,linecolor=blue]{-}{d}{jt}
\ncline[linewidth=1.5pt,linecolor=blue,linestyle=dashed]{-}{jt}{jd}
\ncline[linewidth=1.5pt,linecolor=blue]{-}{jd}{ju}
\ncbar[angle=180,arm=.7,linewidth=1.5pt,linecolor=blue]{-}{ju}{d}
}%\proofnet
}%\subfloat
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subfloat[Successor on Church numerals]{
\label{subfig:PLTS-succ}
\proofnetpagescaled[rowsep=.1,colsep=1]{\zoomdefault}{.4\textwidth}{
\nOut{a}   \\ \\
\nRlin{b} \\ \\
\nRfor{c} \\ \\
\nRlin{d} \\ \\
\nRpa{e} \\ \\
\nRlin{f} \\ \\
\nAx{g} \\ \\
\nLlin{hu} & \nAx{hd} \\ \\
           & \nLlin{iu} & \nAx{id} \\ \\
\nLpa{ju}  & \nLpa{jd}   \\ \\
\nLlin{ku} &            & \nAx{kd} \\ \\
\nLfor{lu} &            & \nCon{ld} \\ \\
%%%
\ncline{b}{a}
  \nbput{\titiNatT{\modn}\linear\titiNatT{\modm}\qquad(\modn\orelLTSS \modm)}
\ncline{c}{b}
  \nbput{\forall\alpha.
         \tim{\modm}{(\alpha\linear\alpha)}\linear\pa{(\alpha\linear\alpha)}}
\ncline{d}{c}
  \nbput{\tim{\modm}{(\alpha\linear\alpha)}\linear\pa{(\alpha\linear\alpha)}}
\ncline{e}{d}
  \nbput{\pa{(\alpha\linear\alpha)}}
\ncline{f}{e}
  \nbput{\alpha\linear\alpha}
\ncline{g}{f}
  \nbput{\alpha}
\ncline{hu}{g}
\nccurve[angleA=135,angleB=45]{hd}{hu}
  \nbput{\alpha}
\ncline{iu}{hd}
\nccurve[angleA=135,angleB=45]{id}{iu}
\ncangles[angleA=180,angleB=-90,armA=.1,armB=.6]{f}{id}
  \nbput{\alpha}
\ncline{ju}{hu}
  \nbput{\alpha\linear\alpha}
\ncline{jd}{iu}
  \nbput{\alpha\linear\alpha}
\ncline{ku}{ju}
  \nbput{\pa{(\alpha\linear\alpha)}}
\nccurve[angleA=135,angleB=0]{kd}{ku}
\ncline{lu}{ku}
  \nbput{\modn{(\alpha\linear\alpha)}\linear\pa{(\alpha\linear\alpha)}}
\nccurve[angleA=135,angleB=-90]{ld}{jd}
  \naput[npos=0.2]{\pa{(\alpha\linear\alpha)}}
\nccurve[angleA=45,angleB=-45]{ld}{kd}
  \nbput{\modn{(\alpha\linear\alpha)}}
\ncangles[angleA=180,angleB=-90,armA=1,armB=.4]{b}{lu}
%   \nbput{\tim{i_m}{(\alpha\linear\alpha)}}
\ncangles[angleA=180,angleB=-90,armA=.9]{d}{ld}
% box border
\ncbar[angle=0,arm=2.5,linewidth=1.5pt,linecolor=blue]{-}{e}{jd}
\ncline[linewidth=1.5pt,linecolor=blue]{-}{jd}{ju}
\ncbar[angle=180,arm=.7,linewidth=1.5pt,linecolor=blue]{-}{ju}{e}
}%\proofnet
}%\subfloat
}


==> fig-complete-path.tex <==
\complexfigure
{An example of maximal path.}
{figure:An example of complete path}
{%%%%%%%%% bs zx.z(bs f.z)I
\proofnetscaled[rowsep=2pt,colsep=50pt]{\zoomdefault}{
\nOut{a} \\ \\
\nAx{b}  \\ \\
\nLlin{c} \\ \\
\nLlin{e} \\ \\
\nCut{g}  && \nAx{f} & \nAx{d} \\ \\
\nRlin{h} &         && \nCon{i}     \\ \\
\nRlin{j} &         && \nCut{lackcut} \\ \\
\nRP{l}   &         && \nRP{k}     \\ \\
\nAx{n}   &         && \nRfor{m}    \\ \\
\nLlin{p} &         && \simplenet{o}{\Pi}  \\ \\
\nLfor{r} & \nAx{q} \\ \\
\nLP{s}   & \nLP{t}\\ \\
%%%
\ncline{b}{a}
  \naput{\rnode{bau}{(\sige,+)}}
\ncline{c}{b}
  \naput{\rnode{cbu}{(\sige,+)}}
\ncline{e}{c}
  \nbput[npos=0.3]{\rnode{ec}{(\sige\stacka,-)}}
  \naput[npos=0.3]{\rnode{ecu}{(\sige\stacko,+)}}
\ncupr{d}{c}
  \nbput{\rnode{dc}{(\sige,+)}}
\ncupr{f}{e}
\ncline{g}{e}
  \nbput[npos=0.3]{\rnode{ge}{(\sige\stacka\stacko,-)}}
  \naput[npos=0.3]{\rnode{geu}{(\sige\stacko\stacko,+)}}
\ncline{h}{g}
  \nbput{\rnode{hg}{(\sige\stacka\stacko,-)}}
  \naput{\rnode{hgu}{(\sige\stacko\stacko,+)}}
\ncup[offsetA=.1]{i}{f}
\ncline{i}{d}
  \nbput{\rnode{id}{(\sige,+)}}
\ncline{j}{h}
  \nbput{\rnode{jh}{(\sige\stacka,-)}}
  \naput{\rnode{jhu}{(\sige\stacko,+)}}
\ncline{lackcut}{i}
  \nbput{\rnode{LACKi}{(\sigr{(\sige)},+)}}
\ncline{l}{j}
  \naput{\rnode{lj}{(\sige,+)}}
\ncline{k}{lackcut}
  \nbput{\rnode{kLACK}{(\sigr{(\sige)},+)}}
\ncline{m}{k}
\ncline{n}{l}
\ncline[nodesepA=0pt]{o}{m}
\ncline{p}{n}
\ncupr{q}{p}
\ncline{r}{p}
\ncline{s}{r}
\ncline{t}{q}
%%% from right arrows to box assumptions
\ncldownup[armA=2cm,armB=0.6cm]{h}{t}
\ncldownup[armA=0.7cm,armB=0.5cm]{j}{s}
  \nbput{\rnode{js}{(\sige,+)}}
%leftmost box border
\abox[linecolor=blue]{2}{l}{s}{t}
% rightmost box border
\abox[linecolor=blue,loopsize=2.5cm,arm=0.5cm]{0}{k}
%arcs between contexts
\nccurve[angleA=90,angleB=-90,linestyle=dashed,linecolor=magenta]{kLACK}{LACKi}
\nccurve[angleA=90,angleB=-90,linestyle=dashed,linecolor=magenta]{LACKi}{id}
\nccurve[angleA=90,angleB=0,linestyle=dashed,linecolor=magenta]{id}{dc}
\nccurve[angleA=180,angleB=90,linestyle=dashed,linecolor=magenta]{dc}{ec}
\ncline[linestyle=dashed,linecolor=magenta]{ec}{ge}
\ncline[linestyle=dashed,linecolor=magenta]{ge}{hg}
\ncline[linestyle=dashed,linecolor=magenta]{hg}{jh}
\nccurve[angleA=180,angleB=90,linestyle=dashed,linecolor=magenta]{jh}{js}
\nccurve[angleA=-90,angleB=-90,linestyle=dashed,linecolor=magenta]{js}{lj}
\ncline[linestyle=dashed,linecolor=magenta]{lj}{jhu}
\ncline[linestyle=dashed,linecolor=magenta]{jhu}{hgu}
\ncline[linestyle=dashed,linecolor=magenta]{hgu}{geu}
\ncline[linestyle=dashed,linecolor=magenta]{geu}{ecu}
\ncline[linestyle=dashed,linecolor=magenta]{ecu}{cbu}
\ncline[linestyle=dashed,linecolor=magenta]{cbu}{bau}
}%proofnet
}%complexfigure


==> fig-dereliction.tex <==
\proofnetcenter[rowsep=.5cm]{
 &\nVoid{out}              & &            &&\nVoid{out2}\\
 &\nDer[_m]{der}         & &\rightarrow &&\simplenet{b2}{\Pi}\\
 &\simplebox{b}{\Pi}       & &            &\nDer[_{\modm_1}]{der2}&&\nDer[_{\modm_k}]{der3}\\
 \nVoid{i1}&\ldots&\nVoid{i2}&            &\nVoid{i3}&\ldots&\nVoid{i4}
 %%%
 \ncline{der}{out} \nbput {A}
 \ncline{b}{der} \nbput {\modm A}
 \ncup[offsetB=2pt]{i1}{b} \naput {{\modm_1}{B_1}}
 \ncup[offsetB=-2pt]{i2}{b} \nbput {{\modm_k}{B_k}}
 %%%
 \ncline{b2}{out2} \nbput {A}
 \ncup[offsetB=2pt]{der2}{b2} \naput{{B_1}}
 \ncup[offsetB=-2pt]{der3}{b2} \nbput{{B_k}}
 \ncline{i3}{der2} \naput {{\modm_1}{B_1}}
 \ncline{i4}{der3} \nbput {{\modm_k}{B_k}}
}


==> fig-embedding-SLL.tex <==
\complexfigure
{The counterexample described in Section~\ref{sec:embedding-SLL}.}
{fig:embedding-SLL}
{\proofnetpagescaled[rowsep=5mm]{\zoomdefault}{\textwidth}{
 &&&&&\nOut{o}\\
 &&&&&\nRtens{t1}\\
 &&&\nRP{pout}&&&\\
 &&&\nRtens{t2}\\
 &&\nRtens{t3}\\
 &\nId{ia1}&&\nId{ib1}&\nId{ia2}&&\nId{ib2}\\
 &\nCon{mux1}\\
 &&\nLtens{lt1}\\
 &&\nLP{lp1}&&\nLP{lp2}\\
 &&&&&\nLtens{lt2}\\
 &&&&&\nCon{mux2}\\
 &&&\nCon{contr}\\
 &&&\nIn{input}\\
 %%%%%%%%%%%%%%%%%%%%%%
 \ncline{t1}{o} \nbput{\left(\ocsymbol\left(\left(\alpha\otimes\beta\right)\otimes\alpha\right)\right)\otimes\beta}
 \ncupl{pout}{t1}
 \ncline{t2}{pout}
 \ncupl{t3}{t2}
 \ncupl{ia1}{t3} \naput{\alpha}
 \ncupr{ib1}{t3} \nbput{\beta}
 \ncupr{ia2}{t2} \nbput{\alpha}
 \ncupr{ib2}{t1} \nbput{\beta}
 \ncline{mux1}{ia1} \naput{\alpha}
 \ncangle[angleA=180,angleB=-90]{lt1}{mux1} \naput{\ocsymbol\alpha}
 \ncangle[angleA=0,angleB=-90]{lt1}{ib1} \nbput{\beta}
 \ncline{lp1}{lt1}
 \ncline{lp2}{ia2} \nbput{\alpha}
 \ncangle[angleA=180,angleB=-90]{lt2}{lp2} \nbput{\ocsymbol\alpha}
 \ncangle[angleA=0,angleB=-90]{lt2}{ib2} \nbput{\beta}
 \ncline{mux2}{lt2}
 \ncup[offsetA=2pt]{contr}{lp1} \naput{\ocsymbol\left(\ocsymbol\alpha\otimes\beta\right)}
 \ncup[offsetA=-2pt]{contr}{mux2} \nbput{\ocsymbol\left(\ocsymbol\alpha\otimes\beta\right)}
 \ncline{input}{contr} \nbput{\ocsymbol\ocsymbol\left(\ocsymbol\alpha\otimes\beta\right)}
 %%%%%%%%%%%%%%%%%%%%%%
%  \abox[armA=2cm]{2}{pout}{lp1}{lp2}
 \ncline[linewidth=3pt]{-}{lp1}{lp2}
 \ncangle[linewidth=3pt,linearc=0,armA=1cm,armB=2cm,angleA=180,angleB=180]{-}{pout}{lp1}
 \ncangle[linewidth=3pt,linearc=0,armA=1cm,armB=0.5cm,angleA=0,angleB=0]{-}{pout}{lp2}
}%\proofnet
}%\complexfigure

==> fig-example-levels.tex <==
\complexfigure
{Two of the 4 possible cases in the reduction ${[\rulePo(\modm)/\rulePi(\modm)]}$.
For clarity reasons, we have drawn all the boxes with one only premise and one only conclusion.}
{fig:example-levels}
{
 \subfloat[${[\rulePo(\modm)/\rulePi(\modm)]}$, with $\modm\in\Y,\modq\in\X$]{
  \proofnetpagescaled{\zoomdefault}{3cm}{
    \nVoid{out}\\
    \nRP[(\modq)]{rp1}\\
    \simplenet{pn1}{\Pi}\\
    \nLP[(\modm)]{lp1}\\
    \nCut{ct}\\
    \nRP[(\modm)]{rp2}\\
    \simplenet{pn2}{\Sigma}\\
    \nLP[(\modn)]{lp2}\\
    \nVoid{in}
    %%%%%%%
    \ncline{rp1}{out}
    \ncline{pn1}{rp1}
    \ncline{lp1}{pn1}
    \ncline{ct}{lp1}
    \ncline{rp2}{ct}
    \ncline{pn2}{rp2}
    \ncline{lp2}{pn2}
    \ncline{in}{lp2}
    %%%%%%%%
    \abox[linecolor=red]{1}{rp1}{lp1}
    \abox[linecolor=blue,linestyle=dashed]{1}{rp2}{lp2}
  }%proofnet
  $\rightarrow$
  \proofnetpagescaled{0.9}{3cm}{
    \nVoid{out}\\
    \nRP[(\modq)]{rp1}\\
    \simplenet{pn1}{\Pi}\\
    \nCut{ct}\\
    \simplenet{pn2}{\Sigma}\\
    \nLP[(\modn)]{lp2}\\
    \nVoid{in}
    %%%%%%%
    \ncline{rp1}{out}
    \ncline{pn1}{rp1}
    \ncline{ct}{pn1}
    \ncline{pn2}{ct}
    \ncline{lp2}{pn2}
    \ncline{in}{lp2}
    %%%%%%%%
    \abox[linecolor=red]{1}{rp1}{lp2}
  }%proofnet
 }%subfloat
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \subfloat[${[\rulePo(\modm)/\rulePi(\modm)]}$, with $\modm\in\X$, $\modq\in\Y$]{
  \proofnetpagescaled{\zoomdefault}{3cm}{
    \nVoid{out}\\
    \nRP[(\modq)]{rp1}\\
    \simplenet{pn1}{\Pi}\\
    \nLP[(\modm)]{lp1}\\
    \nCut{ct}\\
    \nRP[(\modm)]{rp2}\\
    \simplenet{pn2}{\Sigma}\\
    \nLP[(\modn)]{lp2}\\
    \nVoid{in}
    %%%%%%%
    \ncline{rp1}{out}
    \ncline{pn1}{rp1}
    \ncline{lp1}{pn1}
    \ncline{ct}{lp1}
    \ncline{rp2}{ct}
    \ncline{pn2}{rp2}
    \ncline{lp2}{pn2}
    \ncline{in}{lp2}
    %%%%%%%%
    \abox[linecolor=blue,linestyle=dashed]{1}{rp1}{lp1}
    \abox[linecolor=red]{1}{rp2}{lp2}
  }%proofnet
  $\rightarrow$
  \proofnetpagescaled{0.9}{3cm}{
    \nVoid{out}\\
    \nRP[(\modq)]{rp1}\\
    \simplenet{pn1}{\Pi}\\
    \nCut{ct}\\
    \simplenet{pn2}{\Sigma}\\
    \nLP[(\modn)]{lp2}\\
    \nVoid{in}
    %%%%%%%
    \ncline{rp1}{out}
    \ncline{pn1}{rp1}
    \ncline{ct}{pn1}
    \ncline{pn2}{ct}
    \ncline{lp2}{pn2}
    \ncline{in}{lp2}
    %%%%%%%%
    \abox[linecolor=blue,linestyle=dashed]{1}{rp1}{lp2}
  }%proofnet
 }%subfloat
}%complexfigure

==> fig-example-pn.tex <==
\complexfigure
{An example of \pn.}
{fig:nets-example}
{
\centering
\proofnetscaled{\zoomdefault}{
&&\nOut{out}\\
&&\nRlin{v}&&\\
&\nVoid{ul}&\nRP[(\modn)]{po1}&\nVoid{ur}\\
&&\nId{id1}&&&&&&\nWea{wr}\\
&\nVoid{dl}&\nLP[(\modq)]{pi1}&&&&\nVoid{ul3}&&\nRP[(\modn)]{po3}&&\nVoid{ur3}\\
&&\nCut{cut1}&&&&&\nVoid{ul4}&\nRP[(\modm)]{po4}&\nVoid{ur4}\\
\nVoid{ul2}&&\nRP[(\modq)]{po2}&\nVoid{ur2}&&&&&\nId{idd}\\
&\nWea{wl}&\nId{id2}&&&&&\nVoid{dl4}&\nLP[(\modr)]{pin}&\\
\nVoid{dl2}&\nLP[(\modq)]{pp1}&\nLP[(\modq)]{pp2}&&&&\nVoid{dl3}&&\nLP[(\modn)]{pinb}&&\\
&&&&\nCon[_\modq(\modn,\modq)]{yy}\\
&&&&\nIn{i1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\ncline{v}{out} \naput{\modq B\multimap\modn{\modm A}}
	\ncline{id1}{po1} \nbput{\modm A}
	\ncldownup[armA=22mm,armB=5mm]{v}{pp1} \naput{\modq B}
	\ncline{cut1}{pi1} \nbput {\modq{\modm A}}
	\ncline{po3}{wr} \nbput {\modn{\modm A}}
	\ncline{pi1}{id1} \nbput {\modm A}
	\ncline{po4}{po3} \nbput {\modm A}
	\ncline{po2}{cut1} \nbput {\modq{\modm A}}
	\ncline{idd}{po4} \nbput A
	\ncline{pp1}{wl} \nbput B
	\ncline{id2}{po2} \nbput {\modm A}
	\ncline{pin}{idd} %\nbput {\modm A}
	\ncline{pp2}{id2} \nbput {\modm A}
	\ncline{pinb}{pin} \nbput {\modm A}
  \ncline{po1}{v} \nbput {\modn{\modm A}}
  \ncline{i1}{yy} \nbput {\modq{\modm A}}
  \ncup[offsetA=2pt,armB=3mm]{yy}{pp2} \nbput{\modq{\modm A}}
  \ncup[offsetA=-2pt,armB=3mm]{yy}{pinb} \naput{\modn{\modm A}}
  \abox{1}{po1}{pi1}
  \abox{2}{po2}{pp1}{pp2}
  \abox[arm=6mm]{1}{po3}{pinb}
  \abox{1}{po4}{pin}
	}
}  %complexfigure


==> fig-inside-proof-maximality.tex <==
\complexfigure
{The \pn s used in the proof of Theorem~\ref{teo:structure-maximal}}
{fig:proof-maximality}
{
 \subfloat[$\spind{(\Sigma_1\cup\chi_1)}{\modr_1}{\modr_1}$ in $\mathcal P_1$]
 {
 \proofnetpagescaled{\zoomdefault}{3.2cm}{
   \nVoid{out}\\ \\
   \simplebox{b}{\scriptstyle\phantom{P_\modq(\modq,\modq)}}\\ \\
   \nCon[_\modq(\modq,\modq)]{c}\\
   \nVoid{in}
   %%%%
   \ncline[linestyle=dashed]{b}{out} \uput{3mm}[-50](out){\  \modr_1A = \modq A}
   \nccurve[angleA=135,angleB=-135,linestyle=dashed]{c}{b}
   \nccurve[angleA=45,angleB=-45,linestyle=dashed]{c}{b}
   \uput{1cm}[180](c){u_1}
   \uput{6mm}[35](c){\modq A}
   \uput{6mm}[145](c){\modq A}
   \ncline{in}{c} \nbput{\  \modr_1A = \modq A}
  }
 \label{fig:proof-maximality-a}
 }
 \subfloat[$\spind{(\Sigma_2\cup\chi_2)}{\modr_2}{\modr_2}$ in $\mathcal P_2$]
 {
 \proofnetpagescaled{0.8}{2.8cm}{
   \nVoid{out}\\ \\
   \simplebox{b}{\scriptstyle{P_\modq(\modq,\modq)}}\\ \\
   \nCon[\phantom{_\modq(\modq,\modq)}]{c}\\
   \nVoid{in}
   %%%%
   \ncline[linestyle=dashed]{b}{out} \uput{3mm}[-60](out){\modr_2A}
   \uput{10mm}[180](b){b_2}
   \uput{5mm}[70](b){\modq A}
   \uput{9mm}[-35](b){\modq A}
   \uput{9mm}[-145](b){\modq A}
   \nccurve[angleA=135,angleB=-135,linestyle=dashed]{c}{b}
   \nccurve[angleA=45,angleB=-45,linestyle=dashed]{c}{b}
   \uput{1cm}[180](c){u_2}
   \ncline{in}{c} \nbput{\modr_2A}
  }
 \label{fig:proof-maximality-b}
 }
 \subfloat[$\Theta$ from  $\Sigma_1$]
 {
 \proofnetpagescaled{\zoomdefault}{2.8cm}{
   &\nVoid{out}\\ \\
   &\simplebox{b}{\scriptstyle\phantom{P_\modq(\modq,\modq)}}\\ \\
   \nVoid{in1}&&\nVoid{in2} \\
   %%%%
   \ncline[linestyle=dashed]{b}{out} \uput{3mm}[-60](out){\modq A}
   \nccurve[angleA=100,angleB=-135,linestyle=dashed]{in1}{b}
   \nccurve[angleA=80,angleB=-45,linestyle=dashed]{in2}{b}
   \uput{2mm}[145](in1){\modq A}
   \uput{2mm}[35](in2){\modq A}
  }
 \label{fig:proof-maximality-c}
 }
 \subfloat[$\spind{(\Sigma\cup\chi)}{\modr_2}{\modr_2}$ in $\mathcal P$]
 {
 \proofnetpagescaled{\zoomdefault}{3.2cm}{
   \nVoid{out}\\ \\
   \simplenet{b}{\Theta}\\ \\
   \nCon[\phantom{_\modq(\modq,\modq)}]{c}\\
   \nVoid{in}
   %%%%
   \ncline[linestyle=dashed]{b}{out} \uput{3mm}[-60](out){\ \modr_2A}
   \uput{3mm}[60](b){\modq A}
   \uput{8mm}[-35](b){\modq A}
   \uput{8mm}[-145](b){\modq A}
   \nccurve[angleA=135,angleB=-135,linestyle=dashed]{c}{b}
   \nccurve[angleA=45,angleB=-45,linestyle=dashed]{c}{b}
   \ncline{in}{c} \nbput{\ \modr_2A}
  }
 \label{fig:proof-maximality-d}
 }
}%complexfigure

==> fig-lal-dereliction.tex <==
\complexfigure
{ Multiplication proofnet in \LAL\ plus $!$-dereliction \subref{fig:mult-lal-der-bang}
  and in \LAL\ plus $\S$-dereliction \subref{fig:mult-lal-der-par}.
  Notice that $\N$ denotes a different type in the two cases. }
{fig:dereliction-and-multiplication}
{
\subfloat[]{
\centering
	\proofnetpagescaled{\zoomdefault}{0.60\textwidth}{
	\nOut{o}\\
	\nRlin{r1}\\
	\nRlin{r2}\\
	\nLlin{lzero}\\
	\nLlin{lbox} && \simplenet{zero}{0}\\
	\nLfor{for}\\
	& \nOC{box}\\
	& \nLlin{ladd}\\
	& \simplenet{add}{\operatorname{add}}\\
	&&  \nOC{boxin}\\
	%%%
	\ncline{r1}{o} \nbput{{!\N}\multimap\N\multimap\N}
	\ncline{r2}{r1} \nbput{\N\multimap\N}
	\ncline{lzero}{r2} \nbput{\N}
	\ncupr{zero}{lzero} \nbput{\N}
	\ncline{lbox}{lzero} \naput{\N\multimap\N}
	\ncupr{box}{lbox} \nbput{{!}(\N\multimap\N)}
	\ncline{ladd}{box} \nbput{\N\multimap\N}
	\ncline{add}{ladd} \naput{\N\multimap\N\multimap\N}
	\ncup[angleB=-30]{boxin}{ladd} \nbput{\N}
	\ncline{for}{lbox} \naput{{!}(\N\multimap\N)\multimap\N\multimap\N}
	%%%
	\ncldownup[armA=2.1cm]{r1}{boxin} \nbput{!\N}
	\ncldownup[armA=2cm,armB=0.5cm]{r2}{for} \naput{\N}
	%%%
	\abox[armA=1.3cm,linecolor=red]{1}{box}{boxin}
	}
\label{fig:mult-lal-der-bang}
}%subfloat
\subfloat[]{
	\proofnetpagescaled{\zoomdefault}{0.30\textwidth}{
	\nOut{o}\\
	\nRlin{r1}\\
	\nRlin{r2}\\
	\nLlin{lzero}\\
	\nDer{pd} && \simplenet{zero}{0}\\
	\nLlin{lbox}\\
	\nLfor{for}\\
	& \nOC{box}\\
	& \nLlin{ladd}\\
	& \simplenet{add}{\operatorname{add}}\\
	&&  \nOC{boxin}\\
	%%%
	\ncline{r1}{o} \nbput{{!\N}\multimap\N\multimap\N}
	\ncline{r2}{r1} \nbput{\N\multimap\N}
	\ncline{lzero}{r2} \nbput{\N}
	\ncupr{zero}{lzero} \nbput{\N}
	\ncline{lbox}{pd} \naput{{\S}(\N\multimap\N)}
	\ncline{pd}{lzero} \naput{\N\multimap\N}
	\ncupr{box}{lbox} \nbput{{!}(\N\multimap\N)}
	\ncline{ladd}{box} \nbput{\N\multimap\N}
	\ncline{add}{ladd} \naput{\N\multimap\N\multimap\N}
	\ncup[angleB=-30]{boxin}{ladd} \nbput{\N}
	\ncline{for}{lbox} \naput{{!}(\N\multimap\N)\multimap{\S}(\N\multimap\N)}
	%%%
	\ncldownup[armA=2.1cm]{r1}{boxin} \nbput{!\N}
	\ncldownup[armA=2cm,armB=0.5cm]{r2}{for} \naput{\N}
	%%%
	\abox[armA=1.3cm,linecolor=red]{1}{box}{boxin}
	}
\label{fig:mult-lal-der-par}
}%subfloat
}%complexfigure

==> fig-lall-booleans.tex <==
\complexfigure
{Booleans.}
{fig:booleans}{
\centering
\subfloat[\TT]{
 \proofnetpagescaled{\zoomdefault}{3cm}{
  &\nVoid{out}\\
  &\nRfor{rfor}\\
  &\nRlin{lambda1}\\
  &\nRlin{lambda2}\\
  \nWea{weak}&\nAx{ax}\\
  %%%%%%%%%%%%%%%
  \ncline{rfor}{out} \nbput{\B}
  \ncline{lambda1}{rfor} \nbput{\alpha\lin\alpha\lin\alpha}
  \ncline{lambda2}{lambda1} \nbput{\alpha\lin\alpha\lin\alpha}
  \ncline{ax}{lambda2} \nbput{\alpha}
  \ncldownup[armA=10mm]{lambda1}{ax} \nbput[npos=0.5]{\alpha}
  \ncldownup[armA=9mm]{lambda2}{weak} \nbput[npos=0.5]{\alpha}
 }
}%subfigure
\subfloat[\FF]{
 \proofnetpagescaled{\zoomdefault}{3cm}{
  &\nVoid{out}\\
  &\nRfor{rfor}\\
  &\nRlin{lambda1}\\
  &\nRlin{lambda2}\\
  \nWea{weak}&\nAx{ax}\\
  %%%%%%%%%%%%%%%
  \ncline{rfor}{out} \nbput{\B}
  \ncline{lambda1}{rfor} \nbput{\alpha\lin\alpha\lin\alpha}
  \ncline{lambda2}{lambda1} \nbput{\alpha\lin\alpha\lin\alpha}
  \ncline{ax}{lambda2} \nbput{\alpha}
  \ncldownup[armA=10mm]{lambda2}{ax} \nbput[npos=0.5]{\alpha}
  \ncldownup[armA=9mm]{lambda1}{weak} \nbput[npos=0.5]{\alpha}
 }
} %subfig
\subfloat[\mbox{$\BoolDiag[b]$}]{
 \proofnetpagescaled{\zoomdefault}{3cm}{
  \nVoid{out}\\
%   \nRlin{lambda1}\\
  \nAx{ax}\\
  \nLlin{iffalse}\\
  \nLlin{iftrue}\\
  \nLfor{lfor} & \simplenet{t}{\TT\otimes\TT} &\simplenet{f}{\FF\otimes\FF}\\
  \nVoid{input}
  %%%%%%%%%%%%%%%
%   \ncline{lambda1}{out} \nbput{\B\lin\B\otimes\B}
  \ncline{ax}{out} \nbput{\B\otimes\B}
  \ncline{iffalse}{ax} \nbput{\B\otimes\B}
  \ncline{iftrue}{iffalse} \nbput{}
  \ncline{lfor}{iftrue} \nbput{\B[\B\otimes\B]}
  \ncangle[angleA=90,angleB=0,linearc=.2]{t}{iftrue} \nbput[npos=0.5]{\B\otimes\B}
  \ncangle[angleA=90,angleB=0,linearc=.2]{f}{iffalse} \nbput[npos=0.5]{\B\otimes\B}
%   \ncldownup[armA=9mm]{lambda1}{lfor} \nbput[npos=0.5]{\B}
  \ncline{input}{lfor}  \nbput{\B}
 }
} %subfig
}

==> fig-lall-scott-nums.tex <==
\complexfigure
{Binary Scott numerals.}
{fig:scott-bin-num}
{
\centering
\subfloat[\mbox{$\ZD$}]{
\proofnetpagescaled{\zoomdefault}{4cm}{
 \nVoid{out}\\
%  \nRmu{rmu}\\
 \nRfor{rfor}\\
 \nRlin{imp1}\\
 \nRlin{imp2}\\
 \nAx{ax}\\
 &\nWea{weak}\\
 %%%%%%%%%%%%
 \ncline{rfor}{out} \nbput{\ND}
%  \ncline{rfor}{rmu} \nbput{\forall\alpha.\alpha\lin(\B\lin\ND\lin\alpha)\lin\alpha}
 \ncline{imp1}{rfor} \nbput{\alpha\lin(\B\lin\ND\lin\alpha)\lin\alpha}
 \ncline{imp2}{imp1} \nbput{(\B\lin\ND\lin\alpha)\lin\alpha}
 \ncline{ax}{imp2} \nbput{\alpha}
 \ncldownup[armA=2mm]{imp1}{ax} \nbput[npos=3.5]{\alpha}
 \ncldownup[armA=4mm]{imp2}{weak} \nbput[npos=2.5]{\B\lin\ND\lin\alpha}
}
} %subfigure
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subfloat[\mbox{$\SD_0[s]$}]{
\proofnetpagescaled{\zoomdefault}{4.5cm}{
 &\nVoid{out}\\
%  &\nRlin{lambda}\\
%  &\nRmu{rmu}\\
 &\nRfor{rfor}\\
 &\nRlin{imp1}\\
 &\nRlin{imp2}\\
 &\nAx{ax}\\
 &\nLlin{llin}\\
 &\nLlin{llinB}\\
 \nWea{weak} && \nAx{ax2} && \simplenet{net}{\TT}\\ \\
 &&\nVoid{input}
 %%%%%%%%%%%%
%  \ncline{lambda}{out} \nbput{\ND\lin\ND}
 \ncline{rfor}{out} \nbput{\ND}
%  \ncline{rfor}{rmu} \nbput{\forall\alpha.\alpha\lin(\B\lin\ND\lin\alpha)\lin\alpha}
 \ncline{imp1}{rfor} \nbput{\alpha\lin(\B\lin\ND\lin\alpha)\lin\alpha}
 \ncline{imp2}{imp1} \nbput{(\B\lin\ND\lin\alpha)\lin\alpha}
 \ncline{ax}{imp2} \nbput{\alpha}
 \ncline{llin}{ax} \nbput{\alpha}
 \ncline{llinB}{llin} \nbput{\alpha}
 \ncldownup[armA=9mm]{imp1}{weak} \nbput[npos=0.5]{\alpha}
 \ncldownup[armA=8mm]{imp2}{llinB} \naput[npos=2.5]{\B\lin\ND\lin\alpha}
%  \ncldownup[armA=11mm]{lambda}{ax2} \nbput[npos=0.5]{\ND}
 \ncline{input}{ax2} \nbput{\ND}
 \ncangle[angleA=90,angleB=0]{ax2}{llin} \nbput[npos=0.2]{\ND}
 \ncangle[angleA=90,angleB=0]{net}{llinB} \nbput[npos=0.5]{\B}
}
} %subfigure
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subfloat[\mbox{$\SD_1[s]$}]{
        \proofnetpagescaled{\zoomdefault}{4.5cm}{
        &\nVoid{out}\\
        %  &\nRlin{lambda}\\
%         &\nRmu{rmu}\\
        &\nRfor{rfor}\\
        &\nRlin{imp1}\\
        &\nRlin{imp2}\\
        &\nAx{ax}\\
        &\nLlin{llin}\\
        &\nLlin{llinB}\\
        \nWea{weak} && \nAx{ax2} && \simplenet{net}{\FF}\\ \\
        &&\nVoid{input}
        %%%%%%%%%%%%
        %  \ncline{lambda}{out} \nbput{\ND\lin\ND}
        \ncline{rfor}{out} \nbput{\ND}
%         \ncline{rfor}{rmu} \nbput{\forall\alpha.\alpha\lin(\B\lin\ND\lin\alpha)\lin\alpha}
        \ncline{imp1}{rfor} \nbput{\alpha\lin(\B\lin\ND\lin\alpha)\lin\alpha}
        \ncline{imp2}{imp1} \nbput{(\B\lin\ND\lin\alpha)\lin\alpha}
        \ncline{ax}{imp2} \nbput{\alpha}
        \ncline{llin}{ax} \nbput{\alpha}
        \ncline{llinB}{llin} \nbput{\alpha}
        \ncldownup[armA=9mm]{imp1}{weak} \nbput[npos=0.5]{\alpha}
        \ncldownup[armA=8mm]{imp2}{llinB} \naput[npos=2.5]{\B\lin\ND\lin\alpha}
        %  \ncldownup[armA=11mm]{lambda}{ax2} \nbput[npos=0.5]{\ND}
        \ncline{input}{ax2} \nbput{\ND}
        \ncangle[angleA=90,angleB=0]{ax2}{llin} \nbput[npos=0.2]{\ND}
        \ncangle[angleA=90,angleB=0]{net}{llinB} \nbput[npos=0.5]{\B}
        }
} %subfigure
}
%%%%%%%%%%
\complexfigure
{Basic operations over binary Scott numerals.}
{fig:binary-scott-operations}
{
\centering
\subfloat[\texttt{predecessor}.]{
 \proofnetpagescaled{\zoomdefault}{5cm}{
 \nVoid{out}\\
%  \nRlin{lambda}\\
 \nAx{ax1}\\
 \nLlin{appid}\\
 \nLlin{appzero} &&&\nRlin{rlinbool}\\
 &\simplenet{netzero}{\varepsilon}  &&\nRlin{identity}\\ \\
 \nLfor{lfor}&&\nWea{weakbool} &\nAx{axIdentity}\\
%  \nLmu{lmu}\\
 \nVoid{input}\\
 %%%%%%%%%%%%%%%%%
%  \ncline{lambda}{out} \nbput{\ND\lin\ND}
 \ncline{ax1}{out} \nbput{\ND}
 \ncline{appid}{ax1} \nbput{\ND}
 \ncline{appzero}{appid} %\nbput{\ND\lin\ND}
 \ncangle[angleA=90,angleB=0]{netzero}{appzero} \nbput\ND
 \ncline{lfor}{appzero} \nbput[npos=0.2]{\ND\{\ND\}}
%  \ncline{lmu}{lfor} \nbput{T}
%  \ncldownup{lambda}{lmu} \nbput\ND
 \ncline{input}{lfor} \nbput\ND
 %%%%%%right subnet
 \ncangle[angleA=90,angleB=0]{rlinbool}{appid} \nbput{\B\lin\ND\lin\ND}
 \ncline{identity}{rlinbool} \nbput{\ND\lin\ND}
 \ncline{axIdentity}{identity} \nbput{\ND}
 \ncldownup[armA=6mm]{rlinbool}{weakbool} \nbput[npos=0.5]{\B}
 \ncldownup[armA=2mm]{identity}{axIdentity} \nbput[npos=0.5]{\ND}
 }
}
\subfloat[\texttt{conditional}.]{
 \proofnetpagescaled{\zoomdefault}{5cm}{
 \nVoid{out}\\
 \nRlin{lambda1}\\
 \nRlin{lambda2}\\
 \nRlin{lambda3}\\
 \nRlin{lambda4}\\
 \nAx{ax1}\\
 \nLlin{appid}\\
 \nLlin{appzero} &&&\nRlin{rlinbool}\\
 &\nAx{axA}&&\nRlin{rlinb}\\
 &&\nWea{weak}&\nAx{axB} \\
 \nLfor{lfor}&&&\nLlin{app1}\\
%  \nLmu{lmu}
 &&&\nLlin{app2}\\
 &&&\nLfor{lforb} \\ \\
 %%%%%%%%%%%%%%%%%
 \ncline{lambda1}{out} \nbput{\ND\lin\ND\lin\ND\lin\ND\lin\ND}
 \ncline{lambda2}{lambda1} %\nbput{\ND}
 \ncline{lambda3}{lambda2} %\nbput{\ND}
 \ncline{lambda4}{lambda3} \nbput{}
 \ncline{ax1}{lambda4} \nbput{\ND}
 \ncline{appid}{ax1} \nbput{\ND}
 \ncline{appzero}{appid} %\nbput{\ND\lin\ND}
 \ncangle[angleA=90,angleB=0]{axA}{appzero} \nbput\ND
 \ncline{lfor}{appzero} \nbput[npos=0.1]{\ND\{\ND\}}
%  \ncline{lmu}{lfor} \nbput{T}
 \ncldownup[armA=7mm]{lambda1}{lfor} \nbput[npos=0.5]\ND
 %%%%%%right subnet
 \ncangle[angleA=90,angleB=0]{rlinbool}{appid} \nbput{\B\lin\ND\lin\ND}
 \ncloop[angleA=180,angleB=0,armA=4mm,armB=7mm,loopsize=83mm]{lambda4}{app2}
    \nbput[npos=0.5]{\ND}   \nbput[npos=4.5]{\ND}
 \ncloop[angleA=180,angleB=0,armA=5mm,armB=8mm,loopsize=93mm]{lambda3}{app1}
    \nbput[npos=0.5]{\ND}   \nbput[npos=4.5]{\ND}
 \ncldownup[armA=6mm,armB=4mm]{lambda2}{axA} \nbput[npos=0.5]{\ND}
 \ncline{rlinb}{rlinbool} \nbput{}
 \ncline{axB}{rlinb} \nbput\ND
 \ncline{app1}{axB} \nbput{\ND}
 \ncline{app2}{app1} \nbput{}
 \ncline{lforb}{app2} \nbput{\B\{\ND\}}
 \ncldownup[armA=6mm]{rlinb}{weak} \nbput[npos=0.5]{\ND}
 \ncldownup[armA=7mm]{rlinbool}{lforb} \nbput[npos=0.5]\B
 }
}
}


==> fig-moral-predecessor.tex <==
\complexfigure
{$\PLTSS{M}$: the Predecessor on Church numerals, with type
 $\titiNatT{\modn}\linear\titiNatT{\modm}$ for every $\modn\oreleqLTSS \modm$.}
{fig:PLTS-PseudoPredCN}
{% Moral predecessor
\hspace{5mm}
\proofnetpagescaled[rowsep=.1,colsep=1]{\zoomdefault}{.9\textwidth}{
\nOut{a}  \\ \\
\nRlin{b} \\ \\
\nRfor{c} \\ \\
\nRlin{d} \\ \\
\nRpa{eu} \\ \\
\nRlin{fu} \\ \\
\nAx{ax} & \nWea{weak} &&&&&& \nRoc{ed}{\modn} \\ \\
\nLten{lten} &&&&&&& \nRlin{fd} \\ \\
\nLlin{gu} && \nRtens{gd} &&&&& \nRtens{gt} \\ \\
           &  \nCut{hu}   && \nAx{hd} &&& \nAx{ht} && \nAx{hq}\\ \\
           &  \net{iu}{I} &&&&&&& \nLlin{id} & \nAx{it}  \\ \\
\nLpa{ju}  &&&&&&&& \nLtens{jd} \\ \\
\nLlin{ku} &&&&&& \nLoc{kd}{\modm} \\ \\
\nLfor{l} \\ \\
%%%
\ncline{b}{a}
  \nbput{\titiNatT{\modn}\linear\titiNatT{\modm}
         \quad
         (\modn\oreleqLTSS \modm)}
\ncangles[angleA=180,angleB=-90,armA=.9,armB=.2]{b}{l}
\ncline{c}{b}
\ncline{d}{c}
  \nbput{\modm{(\alpha\linear\alpha)}
         \linear
         \pa{(\alpha\linear\alpha)}}
\ncline{eu}{d}
  \nbput{\pa{(\alpha\linear\alpha)}}
\ncangles[angleA=180,angleB=-90,armA=1.1,armB=1.5]{d}{kd}
\ncangles[angleA=90,angleB=0,armA=.5,armB=6.5]{ed}{ku}
\ncline{fu}{eu}  \nbput{\alpha\linear\alpha}
\ncline{fd}{ed}
  \nbput{((\alpha\linear\alpha)\otimes\alpha)
         \linear
         ((\alpha\linear\alpha)\otimes\alpha)}
\ncangles[angleA=180,angleB=-90,armA=.2,armB=1.4]{fu}{hd}
\ncline{ax}{fu}
\ncline{lten}{ax}  \nbput{\alpha}
\ncline{lten}{weak}  	\nbput{\alpha\linear\alpha}
\ncline{gu}{lten}
\nccurve[angleA=135,angleB=45]{gd}{gu}
  \nbput{(\alpha\linear\alpha)\otimes\alpha}
\ncangles[angleA=180,angleB=-90,armA=2,armB=.3]{fd}{jd}
\ncline{gt}{fd} \nbput{(\alpha\linear\alpha)\otimes\alpha}
\ncangle[angleA=90,angleB=180]{hu}{gd}
  \nbput{\alpha\linear\alpha}
\ncangle[angleA=90,angleB=0]{hd}{gd}
  \naput{\alpha}
\ncangle[angleA=90,angleB=180]{ht}{gt} \nbput{\alpha\linear\alpha}
\ncangle[angleA=90,angleB=0]{hq}{gt} \naput{\alpha}
\ncline{iu}{hu}
\ncline{id}{hq}
\nccurve[angleA=135,angleB=45]{it}{id}
\ncline{ju}{gu}
\ncline{jd}{id}
  \nbput{\alpha\linear\alpha}
\ncangle[angleA=0,angleB=-90]{jd}{it}
  \naput{\alpha}
\ncline{ku}{ju}
  \nbput{\pa{(((\alpha\linear\alpha)\otimes\alpha)
              \linear
              ((\alpha\linear\alpha)\otimes\alpha))}}
\ncline{kd}{ht}
  \nbput{\alpha\linear\alpha}
\ncline{l}{ku}
  \nbput{\modn{(((\alpha\linear\alpha)\otimes\alpha)
                  \linear
                  ((\alpha\linear\alpha)\otimes\alpha))}
         \linear
         \pa{(((\alpha\linear\alpha)\otimes\alpha)
              \linear
              ((\alpha\linear\alpha)\otimes\alpha))}}
% left box border
\ncbar[angle=0,arm=5.5,linewidth=1.5pt,linecolor=blue]{-}{eu}{ju}
\ncbar[angle=180,arm=.7,linewidth=1.5pt,linecolor=blue]{-}{ju}{eu}
% righ box border
\ncbar[angle=0,arm=3.8,linewidth=1.5pt,linecolor=red]{-}{ed}{kd}
\ncbar[angle=180,arm=.7,linewidth=1.5pt,linecolor=red]{-}{kd}{ed}
}
} %complexfigure

==> fig-proof-classes.tex <==
\complexfigure
{An example of \pn, whose nodes have been classified as in proof of Lemma~\ref{lm:few-paths}.}
{fig:proof-classes}
{
 \centering
 \proofnetscaled{\zoomdefault}{
    &\nVoid{out}\\
    &\nAx{ax}\\
    &\nCut{ctup}\\
    &\simplebox{b1}{}\\
    &\nCon{cn1}\\
    \nCut{ct}\\
    \simplebox{b2}{}\\
    \nCon{cn2}\\
    &\nCon{cn3}\\
    &\simplebox{b}{b}\\
    %%%%%%%%%%%%%%%%
    \ncline{ax}{out}  \ncput{\pnode{bound2}}
    \ncline{ctup}{ax}
    \ncline{b1}{ctup}
    \ncline[offset=3pt]{cn1}{b1}   \ncput{\pnode{bound1}}
    \ncline[offset=-3pt]{cn1}{b1}
    \ncangle[angleA=90,angleB=-90,armB=3mm]{ct}{cn1}
    \ncline{b2}{ct}
    \ncline[offset=3pt]{cn2}{b2}  \ncput{\pnode{bound0}}
    \ncline[offset=-3pt]{cn2}{b2}
    \ncangle[angleA=90,angleB=-90,offsetA=3pt,armB=3mm]{cn3}{cn2}
    \ncangle[angleA=90,angleB=-90,offsetA=-3pt,offsetB=-15pt,armB=25mm]{cn3}{b1}
    \ncline{b}{cn3}
    %%% indices
    \uput{4mm}[180](ax){2}
    \uput{4mm}[180](ctup){2}
    \uput{10mm}[180](b1){2}
    \uput{4mm}[180](cn1){1}
    \uput{4mm}[180](ct){1}
    \uput{10mm}[180](b2){1}
    \uput{4mm}[180](cn2){0}
    \uput{4mm}[180](cn3){0}
    %%% boundaries
    \ncloop[linewidth=1.5pt,linestyle=dashed,linecolor=magenta,angleA=180,angleB=0,armA=5mm,armB=42mm,loopsize=33mm]{-}
      {bound0}{bound0}
      \nbput[npos=3.9]{\Pi_0}
    \ncloop[linewidth=1.5pt,linestyle=dashed,linecolor=magenta,angleA=180,angleB=0,armA=35mm,armB=25mm,loopsize=63mm]{-}
      {bound1}{bound1}
      \nbput[npos=3.9]{\Pi_1}
    \ncloop[linewidth=1.5pt,linestyle=dashed,linecolor=magenta,angleA=180,angleB=0,armA=40mm,armB=30mm,loopsize=91mm]{-}
      {bound2}{bound2}
      \nbput[npos=3.9]{\Pi_2}
 }
}

==> fig-proof-dang-spindles.tex <==
\complexfigure
{Examples relative the proof of Lemma~\ref{lm:good-dangerous-spindle}.}
{fig:various-chains}
{
 \centering
 \subfloat[$\Sigma$]{
  \proofnetpagescaled[rowsep=2mm]{\zoomdefault}{0.4\textwidth}{
     &\nVoid{out}\\
     &\nRP[(\modm)]{rport}\\
     &\nRtens{rte1}\\
     \nAx{ax1}&&\nAx{ax2}\\
     \nLP[(\modm)]{lport1}&&\nLP[(\modn)]{lport2}\\
     &\nLtens{lte}\\
     &\nCut{cut}\\
     &\nRtens{rte2}\\
     &&\nRP[(\modn)]{rport2}\\
     &&\nRtens{rte3}\\
     \nAx{ax3}&&&\nRP[(\modq)]{rport3}\\
     &\nAx{ax4}&&\nAx{ax5}\\
     &&&\nLP[(\modq)]{lport4}\\
     &&\nLP[(\modn)]{lport3}&\nLP[(\modn)]{lport5}\\
     &\nCon[_\modm(\modm,\modn)]{contr}\\
     &\nVoid{input}&&\nVoid{input2}
     %%%%%%%%%%%%%%%%%%
     \ncline{rport}{out} \nbput{\modm(B\otimes(B\otimes\modq C))}
     \ncline{rte1}{rport} \nbput{B\otimes(B\otimes\modq C)}
     \ncupl{ax1}{rte1}
     \ncupr{ax2}{rte1}
     \ncline{lport1}{ax1}  \nbput{B}
     \ncline{lport2}{ax2}  \naput{B\otimes\modq C}
     %%%%%% box1
     \ncangle[linewidth=1.5pt,angleA=180,angleB=180]{-}{rport}{lport1}
     \ncangle[linewidth=1.5pt,angleA=0,angleB=0]{-}{rport}{lport2}
     \ncline[linewidth=1.5pt]{-}{lport1}{lport2}
     %%%%%%%
     \ncangle[angleA=180,angleB=-90]{lte}{lport1}  \naput{\modm B}
     \ncangle[angleA=0,angleB=-90]{lte}{lport2}  \nbput{\modn(B\otimes\modq C)}
     \ncline{cut}{lte}  \nbput{\modm B\otimes\modn(B\otimes\modq C)}
     \ncline{rte2}{cut}
     \ncupl{ax3}{rte2}  \naput{\modm B}
     \ncupr{rport2}{rte2}
     \ncup[offsetA=2pt,armB=25mm]{contr}{ax3}
     \ncup[offsetA=-2pt,armB=2mm]{contr}{lport3}  \naput{\modn B}
     \ncline{input}{contr}  \nbput{\modm B}
     \ncline{input2}{lport5}  \nbput{\modn\modq C}
     %%%%%% box2
     \ncangle[linewidth=1.5pt,angleA=180,angleB=180,armB=20mm]{-}{rport2}{lport3}
     \ncangle[linewidth=1.5pt,angleA=0,angleB=0,armB=7mm]{-}{rport2}{lport5}
     \ncline[linewidth=1.5pt]{-}{lport3}{lport5}
     %%%%% box3
     \ncangle[linewidth=1.5pt,angleA=180,angleB=180]{-}{rport3}{lport4}
     \ncangle[linewidth=1.5pt,angleA=0,angleB=0]{-}{rport3}{lport4}
     %%%%%%%
     \ncline{rte3}{rport2} \nbput{B\otimes\modq C}
     \ncupl{ax4}{rte3}  \naput{B}
     \ncupr{rport3}{rte3}  \nbput{\modq C}
     \ncline{ax5}{rport3}  \nbput{C}
     \ncline{lport4}{ax5}
     \ncline{lport5}{lport4}
     \ncup{lport3}{ax4}
  }
 \label{fig:various-chains-a}
 }%subfig
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \subfloat[$\Sigma'$]{
  \proofnetpagescaled[colsep=2pt,rowsep=2mm]{\zoomdefault}{0.34\textwidth}{
     &\nVoid{out}\\
     &\nRP[(\modm)]{rport}\\
     &\nRtens{rte1}\\
     \nAx{ax1}&&\nAx{ax2}\\
     \nLP[(\modm)]{lport1}&&\nLP[(\modn)]{lport2}\\
     &&\nCut{cut2}\\
     &&\nRP[(\modn)]{rport2}\\
     &&\nRtens{rte3}\\
     &&\nRP[(\modq)]{rport3}\\
     &\nAx{ax4}&\nAx{ax5}\\
     &&\nLP[(\modq)]{lport4}\\
     &\nLP[(\modn)]{lport3}&\nLP[(\modn)]{lport5}\\
     &\nCon[_\modm(\modm,\modn)]{contr}\\
     &\nVoid{input}&\nVoid{input2}
     %%%%%%%%%%%%%%%%%%
     \ncline{rport}{out} \nbput{\modm(B\otimes(B\otimes\modq C))}
     \ncline{rte1}{rport} \nbput{B\otimes(B\otimes\modq C)}
     \ncupl{ax1}{rte1}
     \ncupr{ax2}{rte1}
     \ncline{lport1}{ax1}  \nbput{B}
     \ncline{lport2}{ax2}  \naput{B\otimes\modq C}
     %%%%%% box1
     \ncangle[linewidth=1.5pt,angleA=180,angleB=180]{-}{rport}{lport1}
     \ncangle[linewidth=1.5pt,angleA=0,angleB=0]{-}{rport}{lport2}
     \ncline[linewidth=1.5pt]{-}{lport1}{lport2}
     %%%%%%%
     \ncline{cut2}{lport2}  \nbput{\modn(B\otimes\modq C)}
     \ncline{rport2}{cut2}
     \ncup[offsetA=2pt,armB=58mm]{contr}{lport1}   \nbput{\modm B}
     \ncline[offset=-2pt]{contr}{lport3}  \nbput{\modn B}
     \ncline{input}{contr}  \nbput{\modm B}
     \ncline{input2}{lport5}  \nbput{\modn\modq C}
     %%%%%% box2
     \ncangle[linewidth=1.5pt,angleA=180,angleB=180,armB=3mm]{-}{rport2}{lport3}
     \ncangle[linewidth=1.5pt,angleA=0,angleB=0,armB=7mm]{-}{rport2}{lport5}
     \ncline[linewidth=1.5pt]{-}{lport3}{lport5}
     %%%%% box3
     \ncangle[linewidth=1.5pt,angleA=180,angleB=180]{-}{rport3}{lport4}
     \ncangle[linewidth=1.5pt,angleA=0,angleB=0]{-}{rport3}{lport4}
     %%%%%%%
     \ncline{rte3}{rport2} \nbput{B\otimes\modq C}
     \ncupl{ax4}{rte3}  \naput{B}
     \ncline{rport3}{rte3}  \nbput{\modq C}
     \ncline{ax5}{rport3}  \nbput{C}
     \ncline{lport4}{ax5}
     \ncline{lport5}{lport4}
     \ncline{lport3}{ax4}
  }
 \label{fig:various-chains-b}
 }%subfig

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \subfloat[$\Sigma^\star$]{
  \proofnetpagescaled[colsep=2pt,rowsep=2mm]{\zoomdefault}{0.31\textwidth}{
     &\nVoid{out}\\
     &\nRP[(\modm)]{rport}\\
     &\nRlin{r1}\\
     \nWea{ax1}&\nAx{axx}&\nWea{ax2}\\
     \nLP[(\modm)]{lport1}&&\nLP[(\modn)]{lport2}\\
     &&\nCut{cut2}\\
     &&\nRP[(\modn)]{rport2}\\
     &&\nRlin{r2}\\
     &&\nAx{ax10}\\
     &\nWea{w21}&\nWea{w22}\\
     &\nLP[(\modn)]{lport3}&\nLP[(\modn)]{lport4}\\
     &\nCon[_\modm(\modm,\modn)]{contr}\\
     &\nVoid{input}&\nVoid{in2}
     %%%%%%%%%%%%%%%%%%
     \ncline{rport}{out} \nbput{\modm A}
     \ncline{r1}{rport}  \nbput{A}
     \ncline{axx}{r1}  \nbput{\gamma}
     \ncldownup{r1}{axx}
     \ncline{lport1}{ax1}  \nbput{A}
     \ncline{lport2}{ax2}  \naput{A}
     %%%%%% box1
     \ncangle[linewidth=1.5pt,angleA=180,angleB=180]{-}{rport}{lport1}
     \ncangle[linewidth=1.5pt,angleA=0,angleB=0]{-}{rport}{lport2}
     \ncline[linewidth=1.5pt]{-}{lport1}{lport2}
     %%%%%%%
     \ncline{cut2}{lport2}  \nbput{\modn A}
     \ncline{rport2}{cut2}
     \ncup[offsetA=2pt,armB=47mm]{contr}{lport1}   \nbput{\modm A}
     \ncline[offset=-2pt]{contr}{lport3}  \nbput{\modn A}
     \ncline{input}{contr}    \nbput{\modm A}
     \ncline{in2}{lport4}    \nbput{\modm A}
     %%%%%% box2
     \ncangle[linewidth=1.5pt,angleA=180,angleB=180]{-}{rport2}{lport3}
     \ncangle[linewidth=1.5pt,angleA=0,angleB=0]{-}{rport2}{lport4}
     \ncline[linewidth=1.5pt]{-}{lport3}{lport4}
     %%%%%%%
     \ncline{r2}{rport2} \nbput{A}
     \ncline{ax10}{r2} \nbput{\gamma}
     \ncldownup{r2}{ax10}
     \ncline{lport3}{w21} \nbput{A}
     \ncline{lport4}{w22} \nbput{A}
  }
  \label{fig:various-chains-star}
 }%subfig
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \subfloat[$\Sigma''$]{
  \proofnetpagescaled[colsep=2pt,rowsep=2mm]{\zoomdefault}{0.31\textwidth}{
     &\nVoid{out}\\
     &\nRP[(\modm)]{rport}\\
     &\nRlin{r1}\\
     &\nAx{axx} \\
     \nWea{ax1}&\nWea{ax2}\\
     \nLP[(\modm)]{lport1}&\nLP[(\modn)]{lport2}\\
     &\nCut{cut2}\\
     &\nRP[(\modn)]{rport2}\\
     &\nRlin{r2}\\
     &\nAx{ax10}\\
     &\nWea{w21}\\
     &\nLP[(\modn)]{lport3}\\
     &\nCon[_\modm(\modm,\modn)]{contr}\\
     &\nVoid{input}
     %%%%%%%%%%%%%%%%%%
     \ncline{rport}{out} \nbput{\modm A}
     \ncline{r1}{rport}  \nbput{A}
     \ncline{axx}{r1}  \nbput{\gamma}
     \ncldownup{r1}{axx}
     \ncline{lport1}{ax1}  \nbput{A}
     \ncline{lport2}{ax2}  \naput{A}
     %%%%%% box1
     \ncangle[linewidth=1.5pt,angleA=180,angleB=180]{-}{rport}{lport1}
     \ncangle[linewidth=1.5pt,angleA=0,angleB=0]{-}{rport}{lport2}
     \ncline[linewidth=1.5pt]{-}{lport1}{lport2}
     %%%%%%%
     \ncline{cut2}{lport2}  \nbput{\modn A}
     \ncline{rport2}{cut2}
     \ncup[offsetA=2pt,armB=47mm]{contr}{lport1}   \nbput{\modm A}
     \ncline[offset=-2pt]{contr}{lport3}  \nbput{\modn A}
     \ncline{input}{contr}    \nbput{\modm A}
     %%%%%% box2
     \ncangle[linewidth=1.5pt,angleA=180,angleB=180,armB=5mm]{-}{rport2}{lport3}
     \ncangle[linewidth=1.5pt,angleA=0,angleB=0,armB=3mm]{-}{rport2}{lport3}
     %%%%%%%
     \ncline{r2}{rport2} \nbput{A}
     \ncline{ax10}{r2} \nbput{\gamma}
     \ncldownup{r2}{ax10}
     \ncline{lport3}{w21} \nbput{A}
     \ncline{lport4}{w22} \nbput{A}
  }
%   \proofnetpagescaled[colsep=2pt]{0.7}{0.31\textwidth}{
%      &\nVoid{out}\\
%      &\nRP[(\modm)]{rport}\\
%      &\nRlin{r1}\\
%      \nWea{ax1}&\nAx{axx}&\nWea{ax2}\\
%      \nLP[(\modm)]{lport1}&&\nLP[(\modn)]{lport2}\\
%      &&\nCut{cut2}\\
%      &&\nRP[(\modn)]{rport2}\\
%      &&\nRlin{r2}\\
%      &&\nAx{ax10}\\
%      &\nWea{w21}\\
%      &\nLP[(\modn)]{lport3}\\
%      &\nCon[_\modm(\modm,\modn)]{contr}\\
%      &\nVoid{input}
%      %%%%%%%%%%%%%%%%%%
%      \ncline{rport}{out} \nbput{\modm A}
%      \ncline{r1}{rport}  \nbput{A}
%      \ncline{axx}{r1}  \nbput{\gamma}
%      \ncldownup{r1}{axx}
%      \ncline{lport1}{ax1}  \nbput{A}
%      \ncline{lport2}{ax2}  \naput{A}
%      %%%%%% box1
%      \ncangle[linewidth=1.5pt,angleA=180,angleB=180]{-}{rport}{lport1}
%      \ncangle[linewidth=1.5pt,angleA=0,angleB=0]{-}{rport}{lport2}
%      \ncline[linewidth=1.5pt]{-}{lport1}{lport2}
%      %%%%%%%
%      \ncline{cut2}{lport2}  \nbput{\modn A}
%      \ncline{rport2}{cut2}
%      \ncup[offsetA=2pt,armB=51mm]{contr}{lport1}   \nbput{\modm A}
%      \ncline[offset=-2pt]{contr}{lport3}  \nbput{\modn A}
%      \ncline{input}{contr}    \nbput{\modm A}
%      %%%%%% box2
%      \ncangle[linewidth=1.5pt,angleA=180,angleB=180]{-}{rport2}{lport3}
%      \ncangle[linewidth=1.5pt,angleA=0,angleB=0,armB=25mm]{-}{rport2}{lport3}
%      %%%%%%%
%      \ncline{r2}{rport2} \nbput{A}
%      \ncline{ax10}{r2} \nbput{\gamma}
%      \ncldownup{r2}{ax10}
%      \ncline{lport3}{w21} \nbput{A}
%      \ncline{lport4}{w22} \nbput{A}
%   }
  \label{fig:various-chains-c}
 }%subfig
}

==> fig-proof-new-criterion.tex <==
\complexfigure
{An example of dangerous spindle $\Sigma$, as in proof of Proposition~\ref{prop:new-criterion}.}
{fig:proof-new-criterion}
{
 \centering
 \subfloat[$\Sigma$]{
 \proofnetpagescaled{\zoomdefault}{6.5cm}{
   &&\nVoid{out}\\
   \nVoid{o0}&&\simplebox{b1}{}\\
   &\nCon{cn1}\\
   \nVoid{o1}&\simplebox{b2}{}&\nVoid{o2}\\
   \nCon{cn2}&&\nCon{cn3}\\
   \nCut{cut1}\\
   \simplebox{b3}{}\\
   &\nCon{cn4}\\
   &\nVoid{input}\\
   %%%%%%%
   \ncline{b1}{out} \nbput{\modq}
   \ncangle[angleA=90,angleB=-90,offsetA=3pt,armB=3mm]{cn1}{o0}
   \ncangle[angleA=90,angleB=-90,offsetA=-3pt,armB=3mm]{cn1}{b1}
   \ncline{b2}{cn1}
   \ncangle[angleA=90,angleB=-90,offsetA=-3pt,offsetB=3pt,armB=3mm]{cn2}{b2}
   \ncline[offset=3pt]{cn2}{o1}
   \ncline{cut1}{cn2} \naput{\modr}
   \ncline{b3}{cut1}
   \ncangle[angleA=90,angleB=-90,offsetA=3pt,armB=3mm,offsetB=-3pt]{cn3}{b2} \nbput{\mods}
   \ncline[offset=-3pt]{cn3}{o2}
   \ncangle[angleA=90,angleB=-90,offsetA=3pt,armB=3mm]{cn4}{b3}
   \ncangle[angleA=90,angleB=-90,offsetA=-3pt]{cn4}{cn3}
   \ncline{input}{cn4} \nbput{\modq}
   %%%%%%%
   \uput{10mm}[0](b1){d}
   \uput{4mm}[0](cn4){u}
 }
 }
 \subfloat[One of the simpler dangerous spindles induced by $\Sigma$.]{
 \proofnetpagescaled{\zoomdefault}{4cm}{
   \nVoid{out}\\
   \simplebox{b}{}\\
   \nCon{c}\\
   \nVoid{input}
   %%%%%%%
   \ncline{b}{out} \nbput{\modq}
   \ncline[offset=3pt]{c}{b} \naput{\modr}
   \ncline[offset=-3pt]{c}{b} \nbput{\mods}
   \ncline{input}{c} \nbput{\modq}
 }
 }
}

==> fig-proofnet-intro.tex <==
\proofnetpagescaled{\zoomdefault}{\textwidth}{
 &&\nVoid{out}\\
 &&\nRtens{rte}\\
 &\nOC{roc}&&\nId{a2}\\
 &\nId{a1}\\
 &\nOC{loc}\\
 \nWea{weak}&&&\nVoid{input2}\\
 &\nCon{cntr}\\
 &\nVoid{input}
 %%%%%%%%%%%
 \ncline{rte}{out}	\nbput{{!A}\otimes B}
 \ncupl{roc}{rte}	\nbput{!A}
 \ncline{a1}{roc}	\nbput{A}
 \ncupr{a2}{rte}	\nbput{B}
 \ncline{loc}{a1}	\nbput{A}
 \ncline{cntr}{loc}	\nbput{!A}
 \ncup[offsetA=2pt]{cntr}{weak}	\naput[npos=2.5]{!A}
 \ncline{input}{cntr}	\nbput{!A}
 \ncline{input2}{a2}	\nbput{B}
 %%%%
 \abox{1}{roc}{loc}
}


==> fig-quasi-connected.tex <==
\complexfigure
{An example of quasi-connected module, with principal premises $\{u_1,u_2\}$ and principal conclusions $\{u_4,u_6,u_7\}$.
Notice that $u_3$ cannot be a principal premise.}
{fig:quasi-connected}
{
 \centering
 \proofnetpagescaled{\zoomdefault}{2cm}{
   \nVoid{o1}&\nVoid{o2}&\nVoid{o3}\\
   &\simplebox{sb}{}\\
   \nCon{c1}&&\nAx{ax}&&\nWea{weak}\\
   \nVoid{i1}&&\nVoid{i2} &&\nVoid{i3}
   %%%%%%%
   \ncline{sb}{o2} \nbput{u_6}
   \ncline[offset=3pt]{c1}{o1} \nbput{u_4}
   \ncangle[angleA=90,angleB=-90,offsetA=-3pt,armB=3mm]{c1}{sb} \nbput{u_5}
   \ncline{i1}{c1} \nbput{u_1}
   \ncline{ax}{o3} \nbput{u_7}
   \ncline{i2}{ax} \nbput{u_2}
   \ncline{i3}{weak} \nbput{u_3}
 }
}

==> fig-scott-duplication.tex <==
\complexfigure
{The \emph{Duplication} proof net $\DD_M:\ND\lin\ND\otimes\ND$.}
{fig:duplication}
{
 \hspace{2mm}
 \subfloat[$M>0$]{
  \proofnetpagescaled[colsep=5pt]{\zoomdefault}{.6\textwidth}{
  %%% WARNING: subfigure is larger than .6\textwidth,
  %%% so that I get overlapping of subfigures
	       \nVoid{out}\\
	       \nAx{axA}\\
	       \nLlin{llin1}\\
	       &&&\nRlin{rlin1}\\
	       \nLlin{llin2}&&&\nRlin{rlin2}\\
	       &\simplenet{feps}{\varepsilon\otimes\varepsilon}&&\nAx{ax1}\\
	       \nLfor{lforA}&&&\nLlin{appldelta}\\
	       &&&&\simplenet[19mm]{dm}{\DD_{M-1}}\\
	       &&\\
	       &&&\nLlin{appl1}\\
	       &&&\nLlin{appl0}\\
	       &&&\nLfor{lfor}&&\nRlin{rs0}&&&&\nRlin{rs1}\\
	       &&&&&\nRtens{rte0}&&&&\nRtens{rte1}\\
	       &&&&\simplenet{s0a}{\texttt{succ}_0}&&\simplenet{s0b}{\texttt{succ}_0}&&\simplenet{s1a}{\texttt{succ}_1}&&\simplenet{s1b}{\texttt{succ}_1}\\
	       &&&&&\nLtens{lte0}&&&&\nLtens{lte1}\\
	       \nVoid{in}&&&&&\nLlin{ls0}&&&&\nLlin{ls1}\\
	       %%%%%%%%%%%%% left side
	       \ncline{axA}{out} \nbput{\ND\otimes\ND}
	       \ncline{llin1}{axA}
	       \ncline{llin2}{llin1}
	       \ncangle[angleA=90,angleB=0]{feps}{llin2} \nbput{\ND\otimes\ND}
	       \ncline{lforA}{llin2} \naput{\ND\{\ND\otimes\ND\}}
% 	       \ncline{lmuA}{lforA} \naput{T}
	       \ncline{in}{lforA} \nbput{\ND}
	       %%%%%%%%%%%%% right side
	       \ncangle[angleA=90,angleB=0]{rlin1}{llin1} \nbput{\B\lin\ND\lin\ND\otimes\ND}
	       \ncline{rlin2}{rlin1}
	       \ncline{ax1}{rlin2}\nbput{\ND\otimes\ND}
	       \ncline{appldelta}{ax1}
	       \ncline{appl1}{appldelta}
	       \ncline{appl0}{appl1}
	       \ncline{lfor}{appl0} \nbput{\B\{\ND\otimes\ND\lin\ND\otimes\ND\}}
	       \ncangle[angleA=90,angleB=0]{dm}{appldelta} \nbput[npos=0.5]{\ND\otimes\ND}
	       \ncldownup[armA=3mm]{rlin1}{lfor} \nbput[npos=0.5]{\B}
	       \ncldownup[armA=2mm]{rlin2}{dm} \nbput[npos=0.5]{\ND}
	       %%%%%%%%%%%%%% succ 0
	       \ncangle[angleA=90,angleB=0]{rs0}{appl0} \nbput[npos=1.5]{\ND\otimes\ND\lin\ND\otimes\ND}
	       \ncline{rte0}{rs0}
	       \ncupl{s0a}{rte0}
	       \ncupr{s0b}{rte0}
	       \ncangle[angleA=180,angleB=-90]{lte0}{s0a}  \nbput{\ND}
	       \ncangle[angleA=0,angleB=-90]{lte0}{s0b}  \naput{\ND}
	       \ncline{ls0}{lte0}
	       \ncldownup[armA=20mm]{rs0}{ls0}
	       %%%%%%%%%%%%%% succ 1
	       \ncangle[angleA=90,angleB=0]{rs1}{appl1} \nbput[npos=1.5]{\ND\otimes\ND\lin\ND\otimes\ND}
	       \ncline{rte1}{rs1}
	       \ncupl{s1a}{rte1}
	       \ncupr{s1b}{rte1}
	       \ncangle[angleA=180,angleB=-90]{lte1}{s1a}  \nbput{\ND}
	       \ncangle[angleA=0,angleB=-90]{lte1}{s1b}  \naput{\ND}
	       \ncline{ls1}{lte1}
	       \ncldownup[armA=16mm]{rs1}{ls1}
  }
  }%subfigure
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \raisebox{3.3cm}{
  \subfloat[$M=0$: dummy value]{
  \proofnetpagescaled{\zoomdefault}{2cm}{
	\nVoid{out}\\
	\simplenet{dum}{\varepsilon\otimes\varepsilon}\\
	\nWea{weak}\\
	\nVoid{in}\\
	%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\ncline{in}{weak} \nbput{\ND}
	\ncline{dum}{out} \nbput{\ND\otimes\ND}
  }}}
 }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> fig-solal-mo-old.tex <==
\complexfigure
{The recursion \pn\ that can be built in \SOLAL. We assume that $\numnor{n}=\numsafe{s}=1$.}
{fig:solal-mo}
{
 \centering
 \proofnetscaled{0.9}{
   \nOut{out}\\
   \nRP[(\tipa{l}{})]{rp1} &&&&&j<t<i<l\in\N\\
   \nAx{ax1}\\
   \nLlin{llin1}\\
   &\simplenet{g}{g}\\
   \nLP[(\tipa{i}{})]{lp1} & \nLP[(\tioc{t}{})]{lp2} & \nLP[(\tioc{t}{})]{lp3}\\
   \nLlin{llin2}\\
   \nLlin{llin3}\\
   \nLfor{lfor} &&&&\nRP[(\tioc{i}{})]{rpA}    &&&&\nRP[(\tioc{i}{})]{rpB}\\
   \nIn{in1}    &&&&\nLlin{llinA}	       &&&&\nLlin{llinB}\\
		&&&&\simplenet{hA}{h_0}        &&&&\simplenet{hB}{h_1}\\
		&&&&\nLP[(\tipa{t}{})]{lpA1}&\nLP[(\tipa{t}{})]{lpA2}
				               &&&\nLP[(\tipa{t}{})]{lpB1}&\nLP[(\tipa{t}{})]{lpB2}\\
		&&&&\nCut{ct1}&\nCut{ct2}&&&\nCut{ct3}&\nCut{ct4}\\
		&&&&\simplebox[10mm]{p1}{P}&\simplebox[10mm]{p2}{P}&&&\simplebox[10mm]{p3}{P}&\simplebox[10mm]{p4}{P}\\
		&&&&\nCon{c11}&&&&\nCon{c12}\\
   &\nCon{c1}&\nCon{c2}\\
   &&\nCut{coecut}\\
   &\simplenet[18mm]{coe}{\texttt{coerce}}&\simplebox[10mm]{coeP}{P}\\
   &\nIn{inn}&\nIn{ins}\\
   %%%%%%%%%%%%%
   \ncline{rp1}{out}  \nbput{\tipa{l}{\timupa{j}{m}{\tiWordT{j}}}}
   \ncline{ax1}{rp1}
   \ncline{llin1}{ax1}  \nbput{\timupa{j}{m}{\tiWordT{j}}}
   \ncline{lp1}{llin1}
   \ncupr{g}{llin1}  \nbput{\timupa{j}{m}{\tiWordT{j}}}
   \ncline{lp2}{g}  \naput{\tiWordT{j}}
   \ncline{lp3}{g}  \nbput{\timupa{j}{m}{\tiWordT{j}}}
   %%%%%%%%%%%%%
   \abox{3}{rp1}{lp1}{lp2}{lp3}
   %%%%%%%%%%%%%
   \ncline{llin2}{lp1} \naput{\tipa{i}{\left(\timupa{j}{m}{\tiWordT{j}}\li\timupa{j}{m}{\tiWordT{j}}\right)}}
   \ncline{llin3}{llin2}
   \ncline{lfor}{llin3}
   \ncline{in1}{lfor}  \nbput{\tiWordT{i}}
   \ncupr{rpA}{llin3}  \nbput[npos=1.1]{\tioc{i}{\left(\timupa{j}{m}{\tiWordT{j}}\li\timupa{j}{m}{\tiWordT{j}}\right)}}
   \ncupr{rpB}{llin2}  \nbput[npos=1.2]{\tioc{i}{\left(\timupa{j}{m}{\tiWordT{j}}\li\timupa{j}{m}{\tiWordT{j}}\right)}}
   %%%%%%%%%%%%%
   \ncline{ct1}{lpA1}  \naput{\tipa{t}{\tiWordT{j}}}
   \ncline{ct3}{lpB1}  \naput{\tipa{t}{\tiWordT{j}}}
   \ncline{p1}{ct1}
   \ncline{p3}{ct3}
   \ncline{c11}{p1} \naput{\tioc{t}{\tiWordT{j}}}
   \ncline{c11}{p3}
   \ncline{c1}{c11}
   \ncline{c1}{lp2} \naput{\tioc{t}{\tiWordT{j}}}
   \ncline{coe}{c1} \naput{\tioc{t}{\tiWordT{j}}}
   \ncline{inn}{coe} \naput{\tiWordT{j}}
   %%%%%%%%%%%%%
   \ncline{ct2}{lpA2}  \naput{\tipa{t}{\timupa{j}{m}{\tiWordT{j}}}}
   \ncline{ct4}{lpB2}  \naput{\tipa{t}{\timupa{j}{m}{\tiWordT{j}}}}
   \ncline{p2}{ct2}
   \ncline{p4}{ct4}
   \ncline{c12}{p2} \naput{\tioc{t}{\timupa{j}{m}{\tiWordT{j}}}}
   \ncline{c12}{p4}
   \ncline{c2}{c12}
   \ncline{c2}{lp3} \naput{\tioc{t}{\timupa{j}{m}{\tiWordT{j}}}}
   \ncline{coecut}{c2}
   \ncline{coeP}{coecut}  \nbput{\tioc{t}{\timupa{j}{m}{\tiWordT{j}}}}
   \ncline{ins}{coeP} \nbput{\timupa{j}{m+1}{\tiWordT{j}}}
   %%%%%%%%%%%% box A
   \abox{2}{rpA}{lpA1}{lpA2}
   \ncline{llinA}{rpA} \nbput{\timupa{j}{m}{\tiWordT{j}}\li\timupa{j}{m}{\tiWordT{j}}}
   \ncline{hA}{llinA}  \nbput{\timupa{j}{m}{\tiWordT{j}}}
   \ncline{lpA1}{hA}   \naput{\tiWordT{j}}
   \ncline{lpA2}{hA}   \nbput{\timupa{j}{m}{\tiWordT{j}}}
   \ncldownup[offsetB=-8pt]{llinA}{hA}
   %%%%%%%%%%%% box B
   \abox{2}{rpB}{lpB1}{lpB2}
   \ncline{llinB}{rpB} \nbput{\timupa{j}{m}{\tiWordT{j}}\li\timupa{j}{m}{\tiWordT{j}}}
   \ncline{hB}{llinB}  \nbput{\timupa{j}{m}{\tiWordT{j}}}
   \ncline{lpB1}{hB}   \naput{\tiWordT{j}}
   \ncline{lpB2}{hB}   \nbput{\timupa{j}{m}{\tiWordT{j}}}
   \ncldownup[offsetB=-8pt]{llinB}{hB}
 }
 \small
 (*) each $P$ is a box containing an axiom
}%complexfigure

==> fig-solal-mo.tex <==
\complexfigure
{The safe \emph{not necessarily linear} recursion \pn\ in \SOLAL. We assume that $\numnor{n}=\numsafe{s}=1$.}
{fig:solal-mo}
{
 \hspace{-4mm}
 \subfloat[Safe and Linear Recursion]{
  \proofnetpagescaled[colsep=4mm]{\zoomdefault}{.55\textwidth}{
                    &\nVoid{out}\\
                    &\ntiPA{po1}{j}\\
                    &\simplenet[8mm]{ax1}{\Pi}\\
                    &\nLlin{appl1}\\
                    &           &&\nRMtens{couple}\\
                    &           &\simplebox[7mm]{zero}{0}&
\nAx{aaa}&\simplebox[15mm]{sigma}{\Lift{[g]}}\\
                    &           &&\nCon{lt1} &\nCon{lt2}\\
     \nLfor{lfor}   &\ntiPA{p1}{j_0}    &&\ntiPA{p2}{j_1}&\ntiPA{p3}{j}\\
     \nCut{cutrev}  &\nLlin{appl2}&\simplenet{rocA}{\texttt{Step}_1}&\nCut{c4}&\nCut{c5}\\
     \simplenet[15mm]{rev}{\texttt{reverse}}
                    &\nLlin{appl3}&\simplenet{rocB}{\texttt{Step}_0}
					&\simplenet[15mm]{coe1}{\texttt{coerce}}
					&\simplebox[15mm]{quasicoe}{ } \\
    \nVoid{inw}     &&&\nVoid{i1}&\nVoid{i2}
    %%%%%
    \ncline{po1}{out} \nbput{{\timupa{j}{m+2}{(\tiWordT{k})}}}
    \ncline{ax1}{po1} \nbput{{\timupa{j}{m+1}{(\tiWordT{k})}}}
    \ncline{appl1}{ax1} \nbput{A}
    \ncline{p1}{appl1} \nbput{A\lin A}
    \ncangle[angleA=90,angleB=0]{couple}{appl1}
      \nbput{A}
    \ncangle[angleA=90,angleB=180]{zero}{couple}
      \naput{\tioc{j}{(\tiWordT{j_0})}}
    \ncangle[angleA=90,angleB=0]{sigma}{couple}
      \nbput{{\timupa{j}{m+1}{(\tiWordT{k})}}}
    \ncline{p2}{lt1} \naput{\tioc{j}{(\tiWordT{j_1})}}
    \ncline{p3}{lt2} \nbput{\tioc{j}{\timupa{j}{m}{(\tiWordT{k})}}}
    %%%
    \ncline{lt1}{aaa}
    \ncline{aaa}{couple} \naput{\tioc{j}{(\tiWordT{j_1})}}
    \nccurve[angleA=40,angleB=220]{lt1}{sigma} \nbput{\tioc{j}{(\tiWordT{j_1})}}
    %%%
    \nccurve[angleA=160,angleB=-60,linestyle=none]{-}{lt2}{couple}  \ncput[npos=0.6]{\nId{idfloat1}}
    \nccurve[angleA=160,angleB=-60]{lt2}{idfloat1}
    \ncline{idfloat1}{couple}
    \ncline{lt2}{sigma} \nbput{\tioc{j}{\timupa{j}{m}{(\tiWordT{k})}}}
    %%%
    \ncline{i1}{coe1} \nbput[npos=0.3]{\tiWordT{j_1}}
    \ncline{c4}{p2}
    \ncline{coe1}{c4} \nbput{\tipa{j_1}{\tioc{j}{(\tiWordT{j_1})}}}
    \ncline{c5}{p3} \nbput{\tipa{j}{\tioc{j}{\timupa{j}{m}{(\tiWordT{k})}}}}
    \ncline{quasicoe}{c5} 
    \ncline{i2}{quasicoe} \nbput{\timupa{i}{m+2}{(\tiWordT{k})}}
    %%%%% box
    \ncangle[linewidth=1.5pt,linecolor=blue,angleA=180,angleB=180]{-}{p1}{po1}
    \ncline[linewidth=1.5pt,linecolor=blue]{-}{p1}{p2}
    \ncline[linewidth=1.5pt,linecolor=blue]{-}{p2}{p3}
    \ncangle[linewidth=1.5pt,linecolor=blue,angleA=0,angleB=0,armB=15mm]{-}{po1}{p3}
    %%%%%
    \ncline{appl2}{p1}
    \ncline{appl3}{appl2}
    %%%%
    \ncloop[angleA=90,angleB=-90]{lfor}{appl3}
    \ncline{cutrev}{lfor}
      \nbput{\tiWordT{j_0}}
    \ncline{rev}{cutrev}
    \ncline{inw}{rev}
      \nbput{\tiWordT{j_0}}
    %%%
    \ncangles[angleA=90,angleB=45]{rocA}{appl2}  \naput[npos=1.45]{\tioc{j_0}{(A\lin A)}}
    \ncangles[angleA=90,angleB=45]{rocB}{appl3}  \naput[npos=1.45]{\tioc{j_0}{(A\lin A)}}
  }%proofnetpagescaled
 }%subfloat
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \subfloat[$\texttt{Step}_i$]{
 \proofnetpagescaled[colsep=4mm]{\zoomdefault}{.5\textwidth}{
 \\
                         &\nVoid{out}\\
                         &\ntiOC{rocA}{j_0} \\
                         &\nRlin{lambdaA}\\
                         &\nRMtens{rtensA}\\
    \simplebox[15mm]{s0}{\texttt{succ}_i}& \nId{idc}  &\simplebox[15mm]{thetaA}{\Lift{[h_i]}}\\
    \nCon{lt1}         &\nCon{lt2}    &\nCon{lt3}\\
                         &\nLMtens{ltensA}\\ \\
    %%%%%output
    \ncline{rocA}{out}  \nbput{\tioc{j_0}{(A\lin A)}}
    %%%%%box:
    \ncloop[linewidth=1.5pt,linecolor=red,loopsize=58mm,armA=28mm,armB=29mm,angleA=180,angleB=0]{-}{rocA}{rocA}
    \ncldownup[armA=24mm,armB=3mm]{lambdaA}{ltensA}
    \ncline{lambdaA}{rocA}
      \nbput{A\lin A}
    \ncline{rtensA}{lambdaA}
       \nbput{A}
    \ncangle[angleA=180,angleB=-90]{ltensA}{contrS}
    \ncangle[angleA=180,angleB=-90]{ltensA}{lt1} \naput{\tioc{j}{(\tiWordT{j_0})}}
    \ncline{ltensA}{lt2} \naput{\tioc{j}{(\tiWordT{j_1})}}
    \ncline{ltensA}{lt3} \nbput{\tioc{j}{\timupa{j}{m}{(\tiWordT{k})}}}
    \ncangle[angleA=0,angleB=-90,offsetB=-6mm]{ltensA}{thetaA}
      \nbput[npos=0.5]{\timupa{j}{m+1}{(\tiWordT{k})}}
    %%%%
    \ncangle[angleA=90,angleB=180]{s0}{rtensA}
       \naput{\tioc{j}{(\tiWordT{j_0})}}
    %%%%
    \ncline{lt1}{s0} \naput{\tioc{j}{(\tiWordT{j_0})}}
    \ncline{lt1}{thetaA}
    %%%%
    \ncline{idc}{rtensA} \naput{\tioc{j}{(\tiWordT{j_1})}}
    \ncline{lt2}{idc}
    \nccurve[angleA=45,angleB=220]{lt2}{thetaA}
    %%%%
    \nccurve[angleA=170,angleB=-60,linestyle=none]{-}{lt3}{rtensA}  \ncput[npos=0.65]{\nId{idfloat2}}
    \nccurve[angleA=170,angleB=-70]{lt3}{idfloat2}
    \ncline{idfloat2}{rtensA}
    \ncline{lt3}{thetaA}
    %%%%
    \ncangle[angleA=90,angleB=0]{thetaA}{rtensA}
      \nbput[npos=1.5]{\timupa{j}{m+1}{(\tiWordT{k})}}
  }%proofnetpagescaled
 }%subfloat
 
{\small
 where we assume $\numnor{n}=\numnor{s}=1$,
 $\Pi$ is projection of its last argument,
 $\nRMtens{x}{}$ and $\nLMtens{x}{}$ are sequences of $\otimes_{\CR}$ and $\otimes_{\CL}$ nodes resp.,
 \texttt{Step}${}_i$, with $i\in{0,1}$, is on the right, and
     $$A = \tioc{j}{(\tiWordT{j_0})}\otimes\ldots\otimes\tioc{j}{(\tiWordT{j_{\numnor n}})}
      \otimes
      \underbrace{\tioc{j}{\timupa{j}{m}{(\tiWordT{k})}}\otimes\ldots\otimes\tioc{j}{\timupa{j}{m}{(\tiWordT{k})}}}_{\numsafe{s}}
      \otimes
      {\timupa{j}{m+1}{(\tiWordT{k})}}.$$
  }%small
}%complexfigure


==> fig-solal-one-coercion.tex <==
\complexfigure{The \pn s $\ocCoerc{j}{i}{k}$ in \SOLAL, with $j< i$, for any $k$.}
{fig:solal-one-Coerce}
{
\centering
\proofnetpagescaled[rowsep=.1,colsep=1]{\zoomdefault}{.4\textwidth}{%%%%% ocCoerce
\nTB{a}   \\ \\
\nRlin{b} \\ \\
\ntiRoc{c}{i} \\ \\
\nAx{d} \\ \\
\nLlin{eu}&\net{ed}{0} \\ \\
\ntiLpa{f}{j}\\ \\
\nLlin{g} \\ \\
\nLlin{hu}&\ntiRoc{hd}{j}&\ntiRoc{ht}{j} \\ \\
\nLfor{iu}&\net{id}{\texttt{succ}_0}&\net{it}{\texttt{succ}_1} \\ \\
%%%
\ncline{b}{a}
   \nbput{\tiWordT{j}\li \tioc{i}{(\tiWordT{k})}}
\ncline{c}{b}
   \nbput{\tioc{i}{(\tiWordT{k})}}
\ncline{d}{c}
\ncline{eu}{d}
\ncline{f}{eu}
   \nbput{\tiWordT{k}\li\tiWordT{k}}
\ncline{g}{f}
   \naput{\tipa{j}{(\tiWordT{k}\li\tiWordT{k})}}
\ncline{hu}{g}
\ncline{iu}{hu}
%%% application arc inside topmost box
\ncangle[angleA=90
        ,angleB=45
        ,linearc=.1]{ed}{eu}
   \nbput{\tiWordT{k}}
%%% application arcs box
\ncangle[angleA=90
        ,angleB=45
        ,linearc=.1]{hd}{hu}
   \nbput{\tioc{j}{(\tiWordT{k}\li\tiWordT{k})}}
\ncangle[angleA=90
        ,angleB=45
        ,linearc=.1]{ht}{g}
   \naput{\tioc{j}{(\tiWordT{k}\li\tiWordT{k})}}
%%% arcs inside lowewrmost boxes
\ncline{id}{hd}
\ncline{it}{ht}
% %%% abstraction links
\ncangles[angleA=180
         ,angleB=-90
         ,armA=1.5
         ,armB=.4
         ,linearc=.1]{b}{iu}
% upper box border
\ncbar[angle=0,arm=2.1,linewidth=1.5pt,linecolor=red]{-}{c}{f}
\ncbar[angle=180,arm=.3,linewidth=1.5pt,linecolor=red]{-}{f}{c}
% lower boxes border
 \ncloop[loopsize=-1.5
        ,angleA=0
        ,angleB=180
        ,linewidth=1.5pt,linecolor=red]{-}{hd}{hd}
 \ncloop[loopsize=-1.5
        ,angleA=0
        ,angleB=180
        ,linewidth=1.5pt,linecolor=red]{-}{ht}{ht}
}
\normalsize
}


==> fig-spindles-intro.tex <==
\complexfigure
{The structure between $e$ and $f$ is an example of \emph{spindle}.
If the spindle is \emph{dangerous}, it is possible connect it to some $g$ labelled $B=\modm A'$.}
{fig:spindles-intro}
{
 \centering
        \proofnetpagescaled[colsep=.3]{\zoomdefault}{.5\textwidth}{
          &&\quad\nVoid{olast}\\
          &\nVoid{o1}&\ \nGen{d}{\scriptstyle d\ \ }{\ldots}\\
          &&\nCon{v}\\
          &&\nCut{cut}\\
          &&\simplebox{w}{b}&\nVoid{o3}\\
          \nVoid{i1}&\simplebox{b1}{\ }&&\nCon{b2}\\
          &&\nCon{u}\\
          &\nVoid{i2}&\nVoid{in}
          %%%%%%%%%%%%%%%%%
          \ncline{d}{olast} \naput[labelsep=1mm,npos=0.5]{g}
%            \nbput{\modn B}
           \nbput{B}
          \ncline{d}{olast}
          \ncup{v}{o1}
          \ncup[linestyle=dashed,offsetA=-1pt]{v}{d}
          \ncline{cut}{v} \ncput{\rnode{wv}{}}
          \ncline{w}{cut} \ncput{\rnode{wv}{}} \naput[labelsep=1mm,npos=0.6]{f}
          \ncup[linestyle=dashed,offsetB=2pt,offsetA=-1pt,armB=3mm]{b1}{w}
          \ncup[linestyle=dashed,offsetB=-2pt,offsetA=2pt,armB=3mm]{b2}{w}
          \ncline{b2}{o3}
          \ncup[linestyle=dashed,offsetA=1pt,armB=5mm]{u}{b1}
          \ncup[linestyle=dashed,offsetA=-1pt,armB=3mm]{u}{b2} \uput{0.25cm}[200](u)u
          \ncline{in}{u} \ncput{\rnode{inu}{}}
                         \naput[labelsep=1mm,npos=0.3]{e}
                         \nbput[labelsep=1mm,npos=0.3]{\modm A}
          \ncangle[angleA=90,angleB=-90,offsetB=10pt,armB=2mm]{i1}{w}
          \ncline[offset=4pt]{i2}{b1}
          \ncline[offset=7pt]{i2}{b1}
          %%%
          \nccurve[linestyle=dashed,linecolor=magenta,linewidth=2pt,angleA=150,angleB=-150]{-}{inu}{wv} >{\tau}
          \nccurve[linestyle=dashed,linecolor=magenta,linewidth=2pt,angleA=30,angleB=-30]{-}{inu}{wv}< {\rho}
%           \nccurve[linestyle=dashed,linecolor=magenta,linewidth=2pt,angleA=90,angleB=-90]{-}{wv}{d} >{\chi}
          }%proofnet
}

==> fig-spindles.tex <==
\complexfigure
{(a) A \spindle, (b) a chain of two \spindle s.}
{fig:spindle-theta-n}
{
  \subfloat[]{
        \proofnetpagescaled[colsep=.3]{\zoomdefault}{.5\textwidth}{
%           &&\quad\nVoid{olast}\\
%           &\nVoid{o1}&\ \nGen{d}{\scriptstyle d\ \ }{\text{Box-in or } \ruleY}\\
%           &&\nCon{v}\\
%           &&\nCut{cut}\\
          &&\nVoid{out}\\
          &&\simplebox{w}{b}&\nVoid{o3}\\
          \nVoid{i1}&\simplebox{b1}{\ }&&\nCon{b2}\\
          &&\nCon{u}\\
          &\nVoid{i2}&\nVoid{in}
          %%%%%%%%%%%%%%%%%
%           \ncline{d}{olast} \naput[labelsep=1mm,npos=0.5]{g}
%            \nbput{B}
%           \ncline{d}{olast}
%           \ncup{v}{o1}
%           \ncup[linestyle=dashed,offsetA=-1pt]{v}{d}
%           \ncline{cut}{v} \ncput{\rnode{wv}{}}
          \ncline{w}{out} \ncput{\rnode{wv}{}} \naput[labelsep=1mm,npos=0.6]{f}
          \ncup[linestyle=dashed,offsetB=2pt,offsetA=-1pt,armB=3mm]{b1}{w}
          \ncup[linestyle=dashed,offsetB=-2pt,offsetA=2pt,armB=3mm]{b2}{w}
          \ncline{b2}{o3}
          \ncup[linestyle=dashed,offsetA=1pt,armB=5mm]{u}{b1}
          \ncup[linestyle=dashed,offsetA=-1pt,armB=3mm]{u}{b2} \uput{0.25cm}[200](u)u
          \ncline{in}{u} \ncput{\rnode{inu}{}}
                         \naput[labelsep=1mm,npos=0.3]{e}
                         \nbput[labelsep=1mm,npos=0.3]{\modm A}
          \ncangle[angleA=90,angleB=-90,offsetB=10pt,armB=2mm]{i1}{w}
          \ncline[offset=4pt]{i2}{b1}
          \ncline[offset=7pt]{i2}{b1}
          %%%
          \nccurve[linestyle=dashed,linecolor=magenta,linewidth=2pt,angleA=150,angleB=-150]{-}{inu}{wv} >{\tau}
          \nccurve[linestyle=dashed,linecolor=magenta,linewidth=2pt,angleA=30,angleB=-30]{-}{inu}{wv}< {\rho}
%           \nccurve[linestyle=dashed,linecolor=magenta,linewidth=2pt,angleA=90,angleB=-90]{-}{wv}{d} >{\chi}
          }
  \label{fig:spindle}
  }%subfigure
%%%%%%%%
  \subfloat[]{
        \proofnetpagescaled{\zoomdefault}{.4\textwidth}{
        &\nVoid{o1}\\
        &\simplebox{v}{d}\\
        &\simplebox{w}{}&                &\nVoid{o3}\\
        \simplebox{b1}{}&                &\nCon{b2}\\
        \nVoid{i1}&\nCon{u}\\
        &\nCon{con3}\\
        &\nCut{cut}\\
        &\simplebox{b3b}{}\\
        &\simplebox{b3}{}\\
        &               &\simplebox{b4}{}\\
        &\nCon{u2}	&\nVoid{i2}\\
        &\nVoid{in}
        %%%
        \ncline{v}{o1}
        \ncline{w}{v}   \ncput{\rnode{wv}{}} \nbput{\ \ \modp C}
        \ncup[offsetB=1pt,linestyle=dashed,armB=3mm]{b1}{w}
        \ncup[offsetB=-1pt,offsetA=1pt,linestyle=dashed,armB=3mm]{b2}{w}
        \ncup[offsetA=-1pt]{b2}{o3}
        \ncup[linestyle=dashed,offsetA=1pt,armB=5mm]{u}{b1}
        \ncup[linestyle=dashed,offsetA=-1pt,armB=3mm]{u}{b2}
        \ncline{con3}{u}   \ncput{\rnode{b3bu}{}}
        \ncline{cut}{con3}
        \ncloop[angleA=90,angleB=-90,offsetA=-2pt,offsetB=-6pt,armA=2mm,armB=5mm,loopsize=7mm]{con3}{w}
        \ncline[linestyle=dashed]{b3b}{cut} \nbput{\ \ \modn B}
        \ncline{b3}{b3b} \ncput{\rnode{b3b3b}{}}
        \ncup[offsetB=-1pt,linestyle=dashed,armB=3mm]{b4}{b3}
        \ncline[offsetB=1pt,linestyle=dashed]{u2}{b3}
        \ncup[linestyle=dashed,offsetA=-1pt,armB=3mm]{u2}{b4} \uput{0.6cm}[-35](u2)u
        \ncline[offset=1pt]{in}{u2} \ncput{\rnode{inu2}{}} \nbput{\ \ \modm A}
        \ncline[offset=3pt]{i1}{b1}
        \ncline[offset=-3pt]{i2}{b4}
        \ncline[offset=-6pt]{i2}{b4}
        %%%
        \nccurve[linestyle=dashed,linecolor=magenta,linewidth=2pt,angleA=150,angleB=-150]{-}{inu2}{b3b3b}
        \nccurve[linestyle=dashed,linecolor=magenta,linewidth=2pt,angleA=30,angleB=-30]{-}{inu2}{b3b3b}
        \nccurve[linestyle=dashed,linecolor=magenta,linewidth=2pt,angleA=90,angleB=-90]{-}{b3b3b}{b3bu}
        \nccurve[linestyle=dashed,linecolor=magenta,linewidth=2pt,angleA=150,angleB=-150]{-}{b3bu}{wv}
        \nccurve[linestyle=dashed,linecolor=magenta,linewidth=2pt,angleA=30,angleB=-30]{-}{b3bu}{wv}
%         \nccurve[linestyle=dashed,linecolor=magenta,linewidth=2pt,angleA=90,angleB=-90]{-}{wv}{v}
        }
  \label{fig:spindles-chain}
  }%subfigure 
}

==> fig-successor.tex <==
\complexfigure
{$\PLTSS{M}$: the Successor on Church numerals with type $\titiNatT{\modn}\linear\titiNatT{\modm}$ for every $\modn\orelLTSS\modm$.}
{fig:PLTS-SuccCN}
{% SuccessorOnCurchNumerals
\proofnetpagescaled[rowsep=.1,colsep=2]{\zoomdefault}{.9\textwidth}{
\nOut{a}   \\ \\
\nRlin{b} \\ \\
\nRfor{c} \\ \\
\nRlin{d} \\ \\
\nRpa{e} \\ \\
\nRlin{f} \\ \\
\nAx{g} \\ \\
\nLlin{hu} & \nAx{hd} \\ \\
           & \nLlin{iu} & \nAx{id} \\ \\
\nLpa{ju}  & \nLpa{jd}   \\ \\
\nLlin{ku} &            & \nAx{kd} \\ \\
\nLfor{lu} &            & \nCon{ld} \\ \\
%%%
\ncline{b}{a}
  \nbput{\titiNatT{\modn}\linear\titiNatT{\modm}\qquad(\modn\orelLTSS \modm)}
\ncline{c}{b}
  \nbput{\forall\alpha.
         \tim{\modm}{(\alpha\linear\alpha)}\linear\pa{(\alpha\linear\alpha)}}
\ncline{d}{c}
  \nbput{\tim{\modm}{(\alpha\linear\alpha)}\linear\pa{(\alpha\linear\alpha)}}
\ncline{e}{d}
  \nbput{\pa{(\alpha\linear\alpha)}}
\ncline{f}{e}
  \nbput{\alpha\linear\alpha}
\ncline{g}{f}
  \nbput{\alpha}
\ncline{hu}{g}
\nccurve[angleA=135,angleB=45]{hd}{hu}
  \nbput{\alpha}
\ncline{iu}{hd}
\nccurve[angleA=135,angleB=45]{id}{iu}
\ncangles[angleA=180,angleB=-90,armA=.1,armB=.6]{f}{id}
  \nbput{\alpha}
\ncline{ju}{hu}
  \nbput{\alpha\linear\alpha}
\ncline{jd}{iu}
  \nbput{\alpha\linear\alpha}
\ncline{ku}{ju}
  \nbput{\pa{(\alpha\linear\alpha)}}
\nccurve[angleA=135,angleB=0]{kd}{ku}
\ncline{lu}{ku}
  \nbput{\modn{(\alpha\linear\alpha)}\linear\pa{(\alpha\linear\alpha)}}
\nccurve[angleA=135,angleB=-90]{ld}{jd}
  \naput[npos=0.2]{\pa{(\alpha\linear\alpha)}}
\nccurve[angleA=45,angleB=-45]{ld}{kd}
  \nbput{\modn{(\alpha\linear\alpha)}}
\ncangles[angleA=180,angleB=-90,armA=1,armB=.4]{b}{lu}
%   \nbput{\tim{i_m}{(\alpha\linear\alpha)}}
\ncangles[angleA=180,angleB=-90,armA=.9]{d}{ld}
% box border
\ncbar[angle=0,arm=3,linewidth=2pt,linecolor=red]{-}{e}{jd}
\ncline[linewidth=2pt,linecolor=red]{-}{jd}{ju}
\ncbar[angle=180,arm=.7,linewidth=2pt,linecolor=red]{-}{ju}{e}
}
}%complexfigure

==> fig-sum-numerals.tex <==
\complexfigure
{$\PLTSS{M}$: the sum of two Church numerals of type
$\titiNatT{\modn}, \titiNatT{\modm}$ with $\modn\oreleqincoLTSS \modm$ and $\modn\lub \modm\in\LTSS$.}
{fig:PLTS-SumCN}
{% SumOnCurchNumerals
\proofnetpagescaled[rowsep=.1,colsep=1.5]{\zoomdefault}{.9\textwidth}{
\nOut{a}   \\ \\
\nRlin{b} \\ \\
\nRlin{c} \\ \\
\nRfor{d} \\ \\
\nRlin{e} \\ \\
\nRpa{f} \\ \\
\nRlin{g} \\ \\
\nAx{h} \\ \\
\nLlin{iu} &            & \nAx{id} \\ \\
           &            & \nLlin{ju} & \nAx{jd} \\ \\
\nLpa{ku}  &            & \nLpa{kd}   \\ \\
\nLlin{lu} & \nAx{ld}   & \nLlin{lt} & \nAx{lq} \\ \\
\nLfor{mu} &            & \nLfor{md} \\ \\
           &            & \nCon{n} \\ \\
%%%%
\ncline{b}{a}
  \nbput{\titiNatT{\modn}\linear\titiNatT{\modm}\linear\titiNatT{(\modn\lub \modm)}
         \quad
         (\modn\oreleqincoLTSS \modm, \modn\lub \modm\in\LTSS)}
\ncline{c}{b}
  \nbput{\titiNatT{\modm}\linear\titiNatT{(\modn\lub \modm)}}
\ncline{d}{c}
  \nbput{\titiNatT{(\modn\lub \modm)}}
\ncline{e}{d}
  \nbput{{(\modn\lub\modm)}{(\alpha\linear\alpha)}\linear\pa{(\alpha\linear\alpha)}}
\ncline{f}{e}
  \nbput{\pa{(\alpha\linear\alpha)}}
\ncline{g}{f}
  \nbput{\alpha\linear\alpha}
\ncline{h}{g}
  \nbput{\alpha}
\ncline{iu}{h}
\nccurve[angleA=135,angleB=45]{id}{iu}
  \nbput{\alpha}
\ncline{ju}{id}
\nccurve[angleA=135,angleB=45]{jd}{ju}
  \nbput{\alpha}
\ncangles[angleA=180,angleB=-90,armA=.1,armB=.5]{g}{jd}
  \nbput{\alpha}
\ncline{ju}{hu}
\ncline{ku}{iu}
  \nbput{\alpha\linear\alpha}
\ncline{kd}{ju}
%   \nbput{\alpha\linear\alpha}
%   \nbput{\pa{(\alpha\linear\alpha)}}
\ncline{lu}{ku}
\nccurve[angleA=135,angleB=45]{ld}{lu}
\ncline{lt}{kd}
\nccurve[angleA=135,angleB=45]{lq}{lt}
\ncline{mu}{lu}
  \nbput{\modn{(\alpha\linear\alpha)}\linear\pa{(\alpha\linear\alpha)}}
\ncline{md}{lt}
  \nbput{\modm{(\alpha\linear\alpha)}\linear\pa{(\alpha\linear\alpha)}}
\nccurve[angleA=135,angleB=-90]{n}{ld}
  \nbput{{\modn}{(\alpha\linear\alpha)}}
\nccurve[angleA=45 ,angleB=-90]{n}{lq}
  \nbput{\modm{(\alpha\linear\alpha)}}
\ncangles[angleA=180,angleB=-90,armA=1  ,armB=.2]{b}{mu}
\ncangles[angleA=180,angleB=-90,armA=1.1,armB=.3]{c}{md}
\ncangles[angleA=180,angleB=-90,armA=1.2]{e}{n}
  \nbput{{(\modn\lub\modm)}{(\alpha\linear\alpha)}}
% box border
\ncbar[angle=0,arm=3.3,linewidth=1.5pt,linecolor=blue]{-}{f}{kd}
\ncline[linewidth=1.5pt,linecolor=blue]{-}{kd}{ku}
\ncbar[angle=180,arm=.7,linewidth=1.5pt,linecolor=blue]{-}{ku}{f}
}
}%complexfigure

==> linear-details.tex <==
\cleardoublepage
\chapter{Encoding linear functions into \texorpdfstring{$\PLTSS{M}$}{P-M-LTS}} \label{app:Linear details}
\index{Linear Time}
%%%%%%%%%%%%%%%%%%%%%%%%%%
In this Appendix we will list some examples of programming inside $\PLTSS{M}$.
The numerals are represented throught \pn s as the one in Figure~\ref{fig:PLTS-CN}.
In Figure~\ref{fig:PLTS-SuccCN}, \ref{fig:PLTS-PseudoPredCN} and \ref{fig:PLTS-SumCN} there are some basic operations over them.



==> solal-data-basic.tex <==
%%%%%%%%%%%%%%%
\subsection{Basic datatypes}
\label{subsection:Basic datatypes}
We define structure and operations relative to \emph{(sorted unary) naturals}, \emph{(sorted binary) words},
\emph{(sorted) lists}, \emph{pairs} and \emph{tuples} exploiting the higher-order features  of \SOLAL. We shall use them extensively in the course of the definition of $\It{1+\numnor{n}}{\numsafe{s}}{H_0}{H_1}{G}$.
%%%
\paragraph{Sorted unary numerals.}
The type $\tiStringT{i}$ of \textit{sorted unary numerals}, or simply \textit{numerals}, is
$\tiStringT{i}=\forall\alpha.\tioc{i}{(\alpha\li\alpha)}\li\tipa{i}{(\alpha\li\alpha)}$, with $i$ its \emph{sort}.
Each natural naturally corresponds to a closed \pn\ $\judg{\String{n}}{}{\tiStringT{i}}$ in \SOLAL.
In \SOLAL\ we can easily program the closed \pn\ $\typed{\SSucc}{\tiStringT{j}\li\tiStringT{j}}$ that yields the \textit{successor} of argument.
%%%
\paragraph{Sorted binary words.}
The type $\tiWordT{i}$ of \textit{sorted binary words}, or simply \textit{words}, is
$\tiWordT{i}=
\forall\alpha.
\tioc{i}{(\alpha\li\alpha)}\li
\tioc{i}{(\alpha\li\alpha)}\li
\tipa{i}{(\alpha\li\alpha)}$, with $i$ its \emph{sort}.
Each word naturally corresponds to a closed \pn\ $\judg{\Word{w}}{}{\tiWordT{i}}$ in \SOLAL.
In \SOLAL\ we can program standard combinators on words.
$\judg{\WsZ}{}{\tiWordT{j}\li\tiWordT{j}},
 \judg{\WsO}{}{\tiWordT{j}\li\tiWordT{j}}$ are two successors that we can use to set
$\TermsToNets{\Sucz}=\WsZ$ and $\TermsToNets{\Suco}=\WsO$.
$\WsO$ obviously generalizes the successor on strings.
$\WsZ$ must be defined to erase every occurrence of the symbol $0$ to the right hand side of the most significant bit of a word, as in \cite{MurawskiOng00}. This forces every $\Word{w}$, with $w\neq 0$, to have $1$ as its most significant bit.
%%%
$\judg{\Wpred}{}{\tiWordT{j}\li\tiWordT{j}}$ is the predecessor which erases the least significant bit of its argument. We can use it to set $\TermsToNets{\Pred}=\Wpred$.
%%%
Finally, $\judg{\WtoS}{}{\tiWordT{j}\li\tiStringT{j}}$ maps a word $\Word{w}$ to a numeral $\String{n}$ so that $n$ counts the number of bits of $w$.
%%%%%
\paragraph{Sorted lists.}
The type $\tiListT{i}{(A)}$ of \textit{sorted lists} whose elements are of type $A$, or simply \textit{lists of type $A$}, is
$\tiListT{i}{(A)}=\forall \alpha.\tioc{i}{(A\li\alpha\li\alpha)}\li\tipa{i}{(\alpha\li\alpha)}$, with $i$ its \emph{sort}.
% $\{\judg{[\Pi_{1},\ldots,\Pi_{n}]}
%         {\Gamma_1,\ldots,\Gamma_n}
%         {\tiListT{i}(A)}
% \mid n\in\Nat\}$ is a family of \pn s in \SOLAL, given that, for every $1\leq k\leq n$,
% $\judg{\Pi_{k}}{\Gamma_k}{A}$ is a \pn\ of \SOLAL\ as well.
% Every $[\Pi_{1},\ldots,\Pi_{n}]$ in the family is a \emph{list}
% with $\bs cx. c\,M_{\Pi_{1}}( \ldots (c\,M_{\Pi_{n}}\,x) \ldots)$ as companion if $M_{\Pi_k}$ is companion of $\Pi_k$, with $1\leq k\leq n$.
$\Nil$ is the name of the \emph{empty list} $[\ ]$.
%%%
\paragraph{Higher-order pairs and tuples.}
We choose to exploit the expressive power of higher and second-order \formulae\ in \SOLAL\ to represent pairs and tuples.
The type $A\tens B$ of \textit{pairs} is $A\tens B=\forall \gamma.(A\li B\li\gamma)\li\gamma$,
a standard second-order encoding. Its generalization to tuples of $n\geq 1$ elements is
$A_1\tens\ldots\tens A_n=
\forall \gamma.((\li^{n}_{k=1} A_k)\li\gamma)\li\gamma$.
% $\{\judg{\lan\Pi_{1},\ldots,\Pi_{n}\ran}
%         {\Gamma_1,\ldots,\Gamma_n}
%         {A_1\tens\ldots\tens A_n}
% \mid n\in\Nat
%  \}$
% is a family of \pn s in \SOLAL, given that, for every $1\leq k\leq n$,
% $\judg{\Pi_{k}}{\Gamma_k}{A}$ is a \pn\ of \SOLAL\ as well.
% Every
% $\judg{\lan\Pi_{1},\ldots,\Pi_{n}\ran}
%       {\Gamma_1,\ldots,\Gamma_n}
%       {A_1\tens\ldots\tens A_n}$ in the family is a \emph{tuple} with
% $\bs x. x\,M_{\Pi_{1}}\ldots M_{\Pi_{n}}$ as companion  if $M_{\Pi_k}$ is companion of $\Pi_k$, with $1\leq k\leq n$.
$\tens^{n} A$ will abbreviate $A\tens\ldots\tens A$, with $n$ occurrences of $A$.

==> solal-intro-enc.tex <==
%%%%%%%%%%%%
\section{\texorpdfstring{The details on the map from \SRNMM\ to \SOLAL}
		        {The details on the map from SRN= to SOLAL}}
\label{section:Recursive functions of SRN into SOLAL: details}
% Recall that, given a \SRN\ recursive function $f^{1+\numnor{n};\numsafe{s}}$, \textcolor{orange}{as defined in Section~{sec:Expressiveness} (ossia in \SRNMM)},
% with $1+\numnor{n}$ normal and $\numsafe{s}$ safe arguments,
% built on suitable $g, h_0, h_1$,
% Proposition~\ref{proposition:From SRNMM to SOLAL} assures the existence of $\TermsToNets{\cdot}$ as a \pn\ of \SOLAL, such that, for every $j<i$, the type of
% $\TermsToNets{f^{1+\numnor{n};\numsafe{s}}}$ is:
% {\small
% $$
% \tiWordT{j}\li
% (\li_{k=1}^{\numnor{n}}\tiWordT{j})\li
% (\li_{k=1}^{\numsafe{s}}\timupa{i}{3}{\tipa{j}{(\tiWordT{j})}})\li
% \timupa{i}{4}{(\tiWordT{j})}$$}
% %%%
% and $\TermsToNets{f(w,\seq{x}{1}{\numnor{n}};\seq{y}{1}{\numsafe{s}})}$ iterates
% $\TermsToNets{h_0}, \TermsToNets{h_1}$ as many times as the length of $w$, starting from
% $\TermsToNets{g(\seq{x}{1}{\numnor{n}};\seq{y}{1}{\numsafe{s}})}$.
% \par
% Here we detail that
% $\TermsToNets{f^{1+\numnor{n};\numsafe{s}}}$ is the \pn\
% $\It{1+\numnor{n}}{\numsafe{s}}{F_0}{F_1}{G}$ in Figure~\ref{fig:It}, given that
% $F_0, F_1, G$ coincide to
% $\TermsToNets{h_0}, \TermsToNets{h_1}, \TermsToNets{g}$, respectively, with the required type.
% The whole definition of $\It{1+\numnor{n}}{\numsafe{s}}{F_0}{F_1}{G}$ needs quite a lot of programming, the main goal being to exploit the \pn\ $\StoL$ in Figure~\ref{fig:StoL} that allows to build lists that contain the safe arguments of $\TermsToNets{f^{1+\numnor{n};\numsafe{s}}}$ at the correct level. We remark that $\StoL$ in Figure~\ref{fig:StoL} is the one in Figure~\ref{fig:StoL-discussion}, but with a slightly more general type, just for sake of generality.
% \par
We proceed as follows.
Section~\ref{subsection:Basic datatypes} is about the basic data types we shall be using, like words, strings, higher-order tuples, \textit{etc.}.
Section~\ref{subsection:Basic nets} introduces the basic nets, namely combinators for basic operation, like, for example, the coercions, that embed a word inside a certain number of boxes.
Section~\ref{subsection:Configurations and transition function between them} defines configurations, pre-configurations, and the transition function $\CtoC{1+\numnor{n}}{\numsafe{s}}$ at the heart of the virtual machine that implements the recursion unfolding inside \SOLAL.
Finally, Section~\ref{subsection:The iteration}, gives the iteration of the transition function, starting from an initial configuration.
%%%%%%%%%%%%
% \paragraph{\Pn s vs. $\lambda$-terms.}
% In Section~\ref{sec:Expressiveness} we exploited an ML-like functional syntax to suggest ``at glance'' the behavior of the \pn\ $\CtoC{1+\numnor{n}}{\numsafe{s}}$.
% In the coming sections we shall keep adopting the same ``pedagogical'' approach. Every \pn\ $\Pi$ will have its own \emph{$\lambda$-term companion} $M_{\Pi}$ whose mere goal is to give an idea about the behaviour of $\Pi$, by using a, generally, widespread syntax, as compared to the one of the \pn s.
% Specifically, gven a \pn\ $\Pi$ and its companion $M_{\Pi})$ a one-to-one correspondence exist between:
% (a.i) the assumptions of $\Pi$ and the free variables of $M_{\Pi}$,
% (a.ii) the \emph{Right Implication} nodes of $\Pi$ and the $\lambda$-abstractions of $M_{\Pi}$,
% (a.iii) the \emph{Left Implication} nodes of $\Pi$ and the $\lambda$-applications of $M_{\Pi}$.
% \par
% Of course, the level information, related to boxes, are completely invisible inside a $\lambda$-companion. The only way to recover some of them inside the syntax of the $\lambda$-terms is by means of appropriate $\beta$-expansions, which allow to record inside $M_{\Pi}$ the occurrence of a box of $\Pi$.
% We mean that $(\bs z.z\, M_{\Pi_2})M_{\Pi_1}$ can be the companion of the \pn\ in Figure~\ref{fig:net-term-corr-ex}, assuming $M_{\Pi_1}, M_{\Pi_2}$ be the companions of $\Pi_1, \Pi_2$, respectively.
% The dummy abstraction of $z$ allows to somewhat keep the boxes around $\Pi_1$ and $\Pi_2$ separate.
% \par
% Finally, we remark that, for easy of reading, every \pn\ we define will be given with a functional-like structure:
% (b.i) for every \emph{Left Implication}, the argument is the righmost edge, the function the lowermost one, while the result of the application is the topmost edge;
% (b.ii) for every \emph{Right Implication}, the abstracted variable is the leftmost edge, the body the lowermost one, while the root of the function being defined is the uppermost edge.
% %%%
% \complexfigure{A net with $\lambda$-term $(\bs z.zM_{\Pi_2})M_{\Pi_1}$ as its companion.}
% {fig:net-term-corr-ex}
% {
% \scriptsize
% \begin{center}
% \begin{tabular}{c}
% \proofnetpagescaled[rowsep=.1,colsep=.2]{0.75}{0.8\textwidth}{%%%%%%%%% boxes in Pi_M vs applications in M
% \nTB{a}      \\ \\
% \ntiRpa{b}{i}\\ \\
% \nAx{eu}  &         &         &         &         &&&&              &\nCut{co} \\ \\
% \nLlin{fu}&         &\net{ft}{\quad\Pi_2\quad}
%                               &         &         &&&&              &\ntiRpa{do}{k}\\ \\
%           &         &         &         &         &&&&              &\net{eo}{\quad\Pi_1\quad}\\ \\ \\
%           &\ntiLpa{gd}{i_1}
%                     &         &\ntiLpa{gq}{i_n}
%                                         &\ntiLpa{gc}{k}
%                                                  &&&&\ntiLpa{fs}{j_1}
%                                                                     &        &\ntiLpa{fn}{j_m}\\ \\ \\
%           &\nTB{hd} &         &\nTB{hq} &         &&&&\nTB{hs}      &        &\nTB{hn}\\
% % 1st column
% \ncline{b}{a}
% \ncline{eu}{b}
% \ncline{fu}{eu}
% % 2nd column
% \ncline{hd}{gd}
% % 2nd-3rd column
% \ncangle[angleA=90
%         ,angleB=-90
%         ,offsetB=.4
%         ,linearc=.1]{gd}{ft}
% % 4th-3rd column
% \ncangle[angleA=90
%         ,angleB=-90
%         ,offsetB=-.4
%         ,linearc=.1]{gq}{ft}
% % 4th column
% \ncline{hq}{gq}
% % 5th-2nd column
% \ncangle[angleA=90
%         ,angleB=-90
%         ,armB=.7
%         ,linearc=.1]{gc}{fu}
% % 6th column
% \ncline{hs}{fs}
% % 6th-8th column
% \ncangle[angleA=90
%         ,angleB=-90
%         ,offsetB=.4
%         ,linearc=.1]{fs}{eo}
% % 9th-8th column
% \ncangle[angleA=90
%         ,angleB=-90
%         ,offsetB=-.4
%         ,linearc=.1]{fn}{eo}
% % 8th column
% \ncline{do}{co}
% \ncline{eo}{do}
% % 9th column
% \ncline{hn}{fn}
% %%% application arcs
% \ncangle[angleA=90
%         ,angleB=45
%         ,linearc=.1]{ft}{fu}
% %%% cut arc
% \ncangles[angleA=90
%          ,angleB=305
%          ,armA=.3
%          ,armB=1.2
%          ,linearc=.1]{co}{gc}
% % abstraction links
% \ncangles[angleA=180
%          ,angleB=-90
%          ,armA=.2
%          ,linearc=.1]{du}{fu}
% % leftmost box
% \ncbar[angle=0,armB=.2,linewidth=2pt,linecolor=blue]{-}{b}{gc}
% \ncline[linewidth=2pt,linecolor=blue]{-}{gc}{gq}
% \ncline[linewidth=2pt,linecolor=blue,linestyle=dashed]{-}{gq}{gd}
% \ncbar[angle=180,armB=.6,linewidth=2pt,linecolor=blue]{-}{gd}{b}
% % rightmost box
% \ncbar[angle=0,armB=.2,linewidth=2pt,linecolor=blue]{-}{do}{fn}
% \ncline[linewidth=2pt,linecolor=blue,linestyle=dashed]{-}{fn}{fs}
% \ncbar[angle=180,armA=.2,linewidth=2pt,linecolor=blue]{-}{fs}{do}
% }
% \end{tabular}
% \end{center}
% \normalsize
% }


